Synthesizing Power and Area Efficient Image Processing Pipelines on FPGAs using Customized Bit-widths

High-level synthesis (HLS) has received significant attention in recent years, improving programmability for FPGAs. PolyMage is a domain-specific language (DSL) for image processing pipelines that also has a HLS backend to translate the input DSL into an equivalent circuit that can be synthesized on FPGAs, while leveraging an HLS suite. The data at each stage of a pipeline is stored using a fixed-point data type (alpha,beta) where alpha and beta denote the number of integral and fractional bits. The power and area savings while performing arithmetic operations on fixed-point data type is known to be significant over using floating point. In this paper, we first propose an interval-arithmetic based range analysis (alpha-analysis) algorithm to estimate the number of bits required to store the integral part of the data at each stage of an image processing pipeline. The analysis algorithm uses the homogeneity of pixel signals at each stage to cluster them and perform a combined range analysis. Secondly, we propose a software architecture for easily deploying any kind of interval/affine arithmetic based range analyses in the DSL compiler. Thirdly, we propose a new range analysis technique using Satisfiability Modulo Theory (SMT) solvers, and show that the range estimates obtained through it are very close to the lower bounds obtained through profile-driven analysis.We evaluated our bitwidth analysis algorithms on four image processing benchmarks listed in the order of increasing complexity: Unsharp Mask, Down-Up Sampling, Harris Corner Detection and Horn-Schunck Optical Flow. For example, on Optical Flow, the interval analysis based approach showed an 1.4x and 1.14x improvement on area and power metrics over floating-point representation respectively; whereas the SMT solver based approach showed 2.49x and 1.58x improvement on area and power metrics when compared to interval analysis.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = main.tex \


PDF = ${SAMPLES:%.tex=%.pdf}
all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex files/*.tex  code/sobel-codes/*.cpp $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

#main.pdf: samplebody-journals.tex

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> code/harris.code.tex <==
\newpage
\begin{appendices}
\section{Harris Corner Detection PolyMage DSL Code}
\lstset{ %
basicstyle=\rmfamily\scriptsize,
keywordstyle=\textbf,
language=Python,                     % choose the language of the code
numbers=none,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=3pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=false,                    % adds a frame around the code
tabsize=1,                      % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=true,        % sets if automatic breaks should only happen at whitespace
escapeinside={(*}{*)},         % if you want to add a comment within your code
framerule=0pt,
morekeywords={Domain,Function,Interval,Accumulator,Variable,
              Constant,Parameter,Kernel2D,Correlate,Min,Max,Sum,
              Image,Case,Default,Upsample,Downsample,Replicate,
              Reduce, UChar, Char, Float, Double, Int, UInt, 
              Short, UShort, Long, ULong, Condition, Stencil, 
              Accumulate}
}
\begin{lstlisting}[language=python,label={listing:hcd},basicstyle=\scriptsize\ttfamily,frame=lines,captionpos=b,caption=PolyMage 
DSL code for Harris Corner Detection,float=h]
R, C = Parameter(Int, "R"), Parameter(Int, "C")
I = Image(Float, "I", [R+2, C+2])

x, y = Variable("x"), Variable("y")
row, col = Interval(0, R+1, 1), Interval(0, C+1, 1)

c = Condition(x, '>=', 1) & Condition(x, '<=', R) & \
    Condition(y, '>=', 1) & Condition(y, '<=', C)

cb = Condition(x, '>=', 2) & Condition(x, '<=', R-1) & \
     Condition(y, '>=', 2) & Condition(y, '<=', C-1)

Iy = Function(varDom = ([x, y], [row, col]), Float, "Iy")
Iy.defn = [ Case(c, Stencil(I(x, y), 1.0/12, \
                                   [[-1,-2,-1], \
                                    [ 0, 0, 0], \
                                    [ 1, 2, 1]])) ]

Ix = Function(varDom = ([x, y], [row, col]), Float, "Ix")
Ix.defn = [ Case(c, Stencil(I(x, y), 1.0/12, \
                                   [[-1, 0, 1], \
                                    [-2, 0, 2], \
                                    [-1, 0, 1]])) ]

Ixx = Function(varDom = ([x, y], [row, col]), Float, "Ixx")
Ixx.defn = [ Case(c, Ix(x, y) * Ix(x, y)) ]

Iyy = Function(varDom = ([x, y], [row, col]), Float, "Iyy")
Iyy.defn = [ Case(c, Iy(x, y) * Iy(x, y)) ]

Ixy = Function(varDom = ([x, y], [row, col]), Float, "Ixy")
Ixy.defn = [ Case(c, Ix(x, y) * Iy(x, y)) ]

Sxx = Function(varDom = ([x, y], [row, col]), Float, "Sxx")
Syy = Function(varDom = ([x, y], [row, col]), Float, "Syy")
Sxy = Function(varDom = ([x, y], [row, col]), Float, "Sxy")
for pair in [(Sxx, Ixx), (Syy, Iyy), (Sxy, Ixy)]:
    pair[0].defn = [ Case(cb, Stencil(pair[1], 1, \
                                       [[1, 1, 1], \
                                        [1, 1, 1], \
                                        [1, 1, 1]])) ]

Det = Function(varDom = ([x, y], [row, col]), Float, "det")
d = Sxx(x, y) * Syy(x, y) - Sxy(x, y) * Sxy(x, y)
Det.defn = [ Case(cb, d) ]

Trace = Function(varDom = ([x, y], [row, col]), Float, "trace")
Trace.defn = [ Case(cb, Sxx(x, y) + Syy(x, y)) ]

Harris = Function(varDom = ([x, y], [row, col]), Float, "harris")
coarsity = Det(x, y) - 0.04 * Trace(x, y) * Trace(x, y)
Harris.defn = [ Case(cb, coarsity) ]
\end{lstlisting}
\end{appendices}


==> figures/harris_annotated_dag.tex <==
 %\begin{figure}[!hb]
    %\begin{minipage}{0.1\textwidth}
  %  \begin{center}
   
\usetikzlibrary{shapes,arrows}
\usetikzlibrary{matrix, positioning, fit}
\definecolor{forestgreen}{rgb}{0.0, 0.5, 0.0}
%\tikzstyle{block} = [draw, fill=blue!20, rectangle, minimum height=2em, minimum width=2em]
%\tikzstyle{block} = [draw=black, rounded corners, thick, line width=0.3mm, fill=blue!20, rectangle, minimum height=2em, minimum width=2em]
%\tikzstyle{group} = [draw=black!100, dashed, line width=0.2mm, rectangle,
%rounded corners, minimum height=1em, minimum width=1em, inner sep=0.4mm]
%\tikzstyle{textblock} = [draw, fill=blue!20, rectangle, rounded corners]
%\tikzstyle{output} = [draw, fill=blue!20, circle, minimum size=1pt]
%\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
%\tikzstyle{fancynodesqr} =[fill=red!100, text=white, rounded corners, minimum height=4em, minimum width=4em]
%\tikzstyle{fancycircle} =[fill=forestgreen!100, text=white, circle, minimum size=2em]
%\tikzstyle{blueflow} = [blue!100, thick, opacity=0.8]
%\tikzstyle{whitebox} =[fill=white!100, text=black, minimum height = 0.1mm, minimum width = 0.1mm]
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------

\tikzstyle{input} = [draw, thick, circle, minimum size=1.2pt]
\tikzstyle{flowarrow} = [black, opacity=0.75]
\tikzstyle{thickflowarrow} = [rounded corners, line width=0.4mm]
\tikzstyle{fancynodelong} =[draw,text=black, rounded corners, minimum height=2em, minimum width=2em]
\tikzstyle{fancynodelong1} =[draw,text=black, rounded corners, minimum height=2em, minimum width=1.3em]
\tikzstyle{fancynodelong2} =[draw, thick, rounded corners, minimum height=2em, minimum width=1.3em]
\tikzstyle{bitw} = [draw,circle,minimum size=0.01pt, scale=0.4]


    \begin{tikzpicture}[auto, node distance=0.625cm,>=latex', scale=1, 
        transform shape]
        % We start by placing the blocks
        \node [input, name=input] {\textbf{img}};
        \node [fancynodelong, below left=0.7cm of input] (Ix) {\textbf{$I_x$}};
        \node [fancynodelong, below right=0.7cm of input] (Iy) {\textbf{$I_y$}};
        \node [fancynodelong, below left=0.7cm of Ix] (Ixx) {\textbf{$I_{xx}$}};
        \node [fancynodelong, below right=0.7cm of Iy] (Iyy) {\textbf{$I_{yy}$}};
        \node [fancynodelong, below=1.4cm of input] (Ixy) {\textbf{$I_{xy}$}};
        \node [fancynodelong, below=0.7cm of Ixy] (Sxy) {\textbf{$S_{xy}$}};
        \node [fancynodelong, below=0.7cm of Ixx] (Sxx) {\textbf{$S_{xx}$}};
        \node [fancynodelong, below=0.7cm of Iyy] (Syy) {\textbf{$S_{yy}$}};
        \node [fancynodelong1, below=2.8cm of Iy] (trace) {\textbf{$trace$}};
        \node [fancynodelong1, below=2.8cm of Ix] (det) {\textbf{$det$}};
        \node [fancynodelong2, below=1.75cm of Sxy] (Harris) {\textbf{Harris}};
        
        % Annotating with bitwidths

\iffalse
        \node [bitw, right=0.07cm of Ix] (Ixw) {\textbf{a}};
        \node [bitw, right=0.07cm of Iy] (Iyw) {\textbf{a}};
        \node [bitw, right=0.07cm of Ixx] (Ixxw) {\textbf{b}};
        \node [bitw, right=0.07cm of Ixy] (Ixyw) {\textbf{b}};
        \node [bitw, right=0.07cm of Iyy] (Iyyw) {\textbf{b}};
        \node [bitw, right=0.07cm of Sxx] (Sxxw) {\textbf{c}};
        \node [bitw, right=0.07cm of Syy] (Syyw) {\textbf{c}};
        \node [bitw, right=0.07cm of Sxy] (Sxyw) {\textbf{c}};
        \node [bitw, right=0.07cm of det] (detw) {\textbf{d}};
        \node [bitw, right=0.07cm of trace] (tracew) {\textbf{e}};
        \node [bitw, right=0.07cm of Harris] (Harrisw) {\textbf{f}};
\fi

        \draw [->, thickflowarrow] (input) -- (Ix);
        \draw [->, thickflowarrow] (input) -- (Iy);
        \draw [->, thickflowarrow] (Ix) -- (Ixx);
        \draw [->, thickflowarrow] (Ix) -- (Ixy);
        \draw [->, thickflowarrow] (Iy) -- (Ixy);
        \draw [->, thickflowarrow] (Iy) -- (Iyy);
        \draw [->, thickflowarrow] (Ixx) -- (Sxx);
        \draw [->, thickflowarrow] (Iyy) -- (Syy);
        \draw [->, thickflowarrow] (Ixy) -- (Sxy);
        \draw [->, thickflowarrow] (Sxx) -- (det);
        \draw [->, thickflowarrow] (Sxy) -- (det);
        \draw [->, thickflowarrow] (Syy) -- (det);
        \draw [->, thickflowarrow] (Sxx) -- (trace);
        \draw [->, thickflowarrow] (Syy) -- (trace);
        \draw [->, thickflowarrow] (det) -- (Harris);
        \draw [->, thickflowarrow] (trace) -- (Harris);

    \end{tikzpicture}
 %   \end{center}
   % \end{minipage}
%\caption{DAG representation of the Harris Corner Detection algorithm.}
%\label{fig:hdag}
%\end{figure}


==> figures/histogram.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
    \input{./plot_ha_s1}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
    \input{./plot_ha_s2}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
    \input{./plot_ha_s3}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
    \input{./plot_ha_s4}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
    \input{./plot_ha_s5}
    \end{subfigure}

\caption{HCD Stage Histograms}
\label{fig:histogram}
\end{figure}

==> files/ack.tex <==
\section{Acknowledgments}
\label{sec:acknowledgments}
We would like to gratefully acknowledge the Science and Engineering Research Board (SERB), Government of India for funded this research work in part through a grant under its EMR program (EMR/2016/008015).

==> files/background.tex <==
\section{Background}
\label{sec:background}
\begin{figure}[tb]
    \centering
  %  \resizebox{\linewidth}{!}{%
        \overview
   % }%
\vskip 5pt
\caption{PolyMage high-level compilation for FPGAs.}
\label{fig:overview}
\end{figure}
In this section, we briefly explain the architecture of the PolyMage-HLS
compilation framework; and further introduce the basics of interval and
affine arithmetic necessary to understand how range analysis techniques based
on them can be seamlessly integrated into our PolyMage-HLS compiler.
\subsection{PolyMage DSL and Compilation Framework}
In this paper, we use the PolyMage DSL and its compiler infrastructure
to implement and evaluate our automatic bitwidth analysis approach.
The PolyMage compiler infrastructure, when it was first
proposed~\cite{mullapudi2015asplos}, comprised an optimizing
source-to-source translator that generated OpenMP C++ code from an input
PolyMage DSL program. Chugh et al.~\cite{chugh16pact} developed a
backend for PolyMage targeting FPGAs by generating
HLS C++ code. The generated C++ code is translated into a hardware design 
expressed in a Hardware Description Language (HDL) such as VHDL or Verilog
using High Level Synthesis compiler.
Figure~\ref{fig:overview}
shows the entire design flow using the PolyMage-HLS compiler and Xilinx Vivado
tool chain. For syntactic details and code examples, we refer the reader to
the PolyMage webpage~\cite{polymage-web}.

\subsection{Interval and Affine arithmetic}
With interval analysis, one estimates the range of an output
signal $z \leftarrow f\left(x, y\right)$ based on the range of the input signals $x$
and $y$, and the function $f$. For example, if the range of $x$ and $y$ are
$[\low{x},\high{x}]$ and $[\low{y}, \high{y}]$ respectively, and
$z\leftarrow x+y$, then the range of $z$ is
$[\low{x}+\low{y}, \high{x} +\high{y}]$. Such range estimation functions have
to be defined for different operations that are applied iteratively to
obtain the ranges of different intermediate and output signals involved in
the computation. Although interval arithmetic is simple and easy
to use in to practice, it suffers from the problem of range over-estimation.
For example, if the range of a signal $x$ is $[5, 10]$, then the interval
arithmetic estimates the range of the expression $x - x$ as $[-5, 5 ]$ whereas
the actual range is $[0, 0]$. This is due to the fact that the interval
arithmetic ignores the correlations between the operand signals if there were any.
%
\iffalse
 Let the range of the two input signals $x$
and $y$ be $[\low{x}, \high{x}]$ and $[\low{y}, \high{y}]$ respectively. Then
range of the resulting signal  $z = x~op~y$  where $op\in\{+,-,*,/, \verb|^| \}$ is
obtained by applying standard rules of interval arithmetic as follows.
\begin{enumerate}
\item {$\mathbf{z=x+y:}$}  $[\low{z},\high{z}] = [\low{x}+\low{y}, \high{x}+\high{y}]$
\item {$\mathbf{z=x-y:}$}  $[\low{z},\high{z}] = [\low{x}-\high{y}, \high{x}-\low{y}]$
\item {$\mathbf{z=x*y:}$} $[\low{z},\high{z}] = [t_1, t_2 ]$  where \\$t_1 = \min\left(\low{x}\low{y}, \low{x}\high{y}, \high{x}\low{y}, \high{x}\high{y}\right)$
and \\ $t_2 = \max\left(\low{x}\low{y}, \low{x}\high{y}, \high{x}\low{y}, \high{x}\high{y}\right)$.
\item $\mathbf{z=x/y:}$$[\low{z},\high{z}] = [\low{x}, \high{x}] * [1/\high{y}, 1/\low{y}]$ if $0 \not \in [\low{y}, \high{y}]$
\item $\mathbf{z = x^n}$
\begin{enumerate}
  \item $n$ is odd: $[\low{z},\high{z}] = [\low{x}^n, \high{x}^n ]$
  \item $n$ is even :
  $\begin{aligned}[t]
  [\low{z},\high{z}] & = & [\low{x}^n, \high{x}^n ] ~\textrm{if}~\low{x} \geq 0 \\
                      & = & [\high{x}^n, \low{x}^n ] ~\textrm{if}~\high{x} < 0\\
                      & = & [0, max\{\low{x}^n, \high{x}^n\} ]~\textrm{otherwise}
  \end{aligned}$
\end{enumerate}
%
\iffalse
   \begin{enumerate}
   \item {\bf If} $\mathbf{\low{y} > 0}$ {\bf or} $\mathbf{\high{y}<0}$: \\$[\low{z},\high{z}] = [t_1, t_2 ]$ where \\ $t_1 = \min\left(\low{x}\mbox{\small/}\low{y}, \low{x}\mbox{\small/}\high{y}, \high{x}\mbox{\small/}\low{y}, \high{x}\mbox{\small/}\high{y}\right)$ and \\$t_2 = \max\left(\low{x}\mbox{\small/}\low{y}, \low{x}\mbox{\small/}\high{y}, \high{x}\mbox{\small/}\low{y}, \high{x}\mbox{\small/}\high{y}\right)$.
   \item {\bf Otherwise:} $[\low{z}, \high{z}] = [\low{p}, \high{p}]$ where $\low{p}$ and $\high{p}$ are obtained via profiling information as explained in Section~\ref{sec:profile}.
   \end{enumerate}
\fi
\end{enumerate}

Note that if an operand $x$ (or $y$) is constant, we get a tight range for
the result since $x=\low{x}=\high{x}$. In the above four cases, division
operation requires special care. If $0$ is present in the range $[\low{y},
\high{y}]$ of the denominator, then the theoretical range of $z$ can
potentially tend to infinity. Although interval arithmetic is simple and easy
to use in practice, it suffers from the problem of range over-estimation.
For example, if the range of a signal $x$ is $[5, 10]$, then the interval
arithmetic estimates the range of the expression $x - x$ as $[-5, 5 ]$ whereas
the actual range is $[0, 0]$. This is due to the fact that the interval
 arithmetic ignores the correlation between the operand signals if there is
 any.
\fi

With affine arithmetic analysis, a signal $x$ is
represented in an affine form as $x=x_0 + \sum_{i=1}^{n} x_i \epsilon_i$
where $\epsilon_i \in [-1, 1]$ are interpreted as independent noise signals
and their respective coefficients $x_i$'s are treated as the weights
associated with them. The interval of the signal $x$ from its affine form
can be inferred as $[x_0-r, x_0+r]$ where $r=\sum_{i=1}^{n} |x_i|$. The
 addition
and subtraction operations on two input signals is defined as
$z=x\pm y = \left(x_0 \pm y_0\right) + \sum_{i=1}^{n}
\left(x_i \pm y_i\right)\epsilon_i$ and yields the resulting signal in its affine form.
The correlation between the signals
$x$ and $y$ is captured by sharing the independent noise signals $\epsilon_i,
1\leq i \leq n $ in their affine forms either partially or totally.
Now, when we perform a computation $x-x$ by considering the signal $x$ in its
affine form, the resulting range will be zero as against the over-estimated
range which we get in interval arithmetic analysis. Thus the techniques based
on affine arithmetic
arrive at better bounds when compared with interval analysis based techniques by
taking into account cancellation effects in computations involving
correlated signals.
However, note that if the operation is multiplication,
then the resulting signal contains quadratic terms and hence has to be
approximated to an affine form. A detailed discussion on affine arithmetic
analysis is beyond the scope of this paper and we recommend the reader to
Stolfi and Figueiredo~\cite{TEMA352} for the same.


==> files/bitwidth.tex <==
\section{Bitwidth Analysis}\label{sec:bitwidth}
In this section, we present the main technical contributions of this paper which
are summarized below.
\begin{enumerate}
\item A simple interval arithmetic based range analysis algorithm
illustrating how DSLs facilitate practical and efficient program analysis
techniques when compared with C/C++ kind of languages
(Section~\ref{sec:ra}).
\item  A software architecture for range analysis in DSL compilers in which variants of interval and affine arithmetic based approaches
can be easily deployed (Section~\ref{sec:ca}).
\item An SMT solver based approach for range analysis
which substantially improves the accuracy of range estimates and contains the
propagation of estimation errors across iterations. Again, such an SMT solver 
based approach would have been hard to realize if not for the DSL compiler 
framework (Section~\ref{sec:smt}).
\item A profile driven approach for range analysis (Section~\ref{sec:profile}).
\item A greedy heuristic search technique for precision estimation
(Section~\ref{sec:precision}).
\end{enumerate}

\subsection{Variable Width Fixed-Point Data Types}
A fixed-point data type is specified by a tuple $(\alpha, \beta)$ where
$\alpha$ and $\beta$ denote the number of bits  allocated for representing
the integral and fractional parts respectively. The total bitwidth of the
data type is $\alpha + \beta$. The decimal value associated with a
fixed-point binary number $x=b_{\alpha-1}\ldots b_0 . b_{-1} \ldots
b_{-\beta}$ depends on whether it is interpreted as an unsigned integer or a
two's complement signed  integer, and is given as follows:
\begin{equation*}
value(x) = \begin{cases}
\sum^{\alpha-1}_{i=-\beta} 2^i b_i & \text{unsigned} \\
-2^{\alpha-1} b_{\alpha-1} + \sum_{i=-\beta}^{\alpha-2} 2^i b_i & \text{2's
    complement.}
\end{cases}
\end{equation*}
This gives us the ranges $[0, 2^{\alpha}-2^{-\beta}]$ and $[-2^{\alpha-1} ,
2^{\alpha-1}-2^{-\beta}]$ for unsigned and signed fixed-point numbers
respectively. The parameter $\alpha$ gives the range of values that can be
represented and the parameter $\beta$ indicates that the values in the range
can be represented at a resolution of $2^{-\beta}$. Hence, the range and
precision can be improved, by increasing $\alpha$ and $\beta$ respectively.
In this paper, we overload the term precision to also mean the entire data
type $(\alpha, \beta)$, and this can be disambiguated based on context.

Fixed-point data types are useful in image processing applications where the
range of values produced during computations is usually limited
and the precision requirements are less demanding  when compared to many
other numerical algorithms. The data type (range and precision) requirement
at a stage depends on the input data type and the nature of local
computations carried out at that particular stage. Further, overflows during
computations can be addressed by using saturation mode arithmetic instead of
the conventional wrap around arithmetic operations performed in CPUs and GPUs.
\iffalse
This feature is
particularly useful in handling image processing pipelines using the
approximate computing paradigm.
\fi
 The complexity of arithmetic operations on
fixed-point data type $(\alpha, \beta)$ is very similar to that of integer
operations on bitwidth $\alpha+\beta$.

\subsection{Range ($\alpha$) Analysis Algorithm}\label{sec:ra}
The number of integer bits required at a stage $I$ denoted as $\alpha_I$ is
a direct function of the bitwidth of the input data and the operations it
performs on them. The input data here refers to the data supplied to the
stage by its predecessor stages in the DAG. Further, the computations on
the pixel signals at each stage of DAG are identical and hence their
corresponding ranges would be the same. This information is implicitly provided
by a PolyMage DSL program and is hard to elicit from C like programs.
We use this insight to group all the pixel signals at a stage and perform a
combined range analysis using interval arithmetic. If the range of the
data produced at a stage is $[\low{x}, \high{x}]$, then the number of
integral bits $\alpha_I$ required to store the data without overflow is as
follows:
\begin{equation*}
%\resizebox{0.9\hsize}{!}{%
    \alpha=
\begin{cases}
    \max(\ceil{\log_2(\ceil{|\low{x}|})},\ceil{\log_2(\floor{|\high{x}|}+1)})+1 & \text{if } \low{x} <0\\
    \ceil{\log_2(\floor{\high{x}}+1)},              & \text{otherwise}.
\end{cases}%
%}
\end{equation*}
The number of fractional bits
$\beta_I$ required at a stage depends on the application-specific error
tolerance or quality metric, and we propose a profile-driven estimation
technique in Section~\ref{sec:profile}.

The range analysis algorithm iterates over the stages of a DAG in a
topologically sorted order. At each stage, an equivalent expression tree
for the computations (point-wise or stencil) is built. Then the range of the
pixel signals is estimated by recursively performing interval arithmetic on the
expression tree using one of following five interval arithmetic rules.
\begin{enumerate}
\item {$\mathbf{z=x+y:}$}  $[\low{z},\high{z}] = [\low{x}+\low{y}, \high{x}+\high{y}]$
\item {$\mathbf{z=x-y:}$}  $[\low{z},\high{z}] = [\low{x}-\high{y}, \high{x}-\low{y}]$
\item {$\mathbf{z=x*y:}$} $[\low{z},\high{z}] = [t_1, t_2 ]$  where \\$t_1 = \min(\low{x}\low{y}, \low{x}\high{y}, \high{x}\low{y}, \high{x}\high{y})$
and \\ $t_2 = \max(\low{x}\low{y}, \low{x}\high{y}, \high{x}\low{y}, \high{x}\high{y})$.
\item $\mathbf{z=x/y:}$$[\low{z},\high{z}] = [\low{x}, \high{x}] * [1/\high{y}, 1/\low{y}]$ if $0 \not \in [\low{y}, \high{y}]$
\item $\mathbf{z = x^n}$
\begin{enumerate}
  \item $n$ is odd: $[\low{z},\high{z}] = [\low{x}^n, \high{x}^n ]$
  \item $n$ is even :
  $\begin{aligned}[t]
  [\low{z},\high{z}] & = & [\low{x}^n, \high{x}^n ] ~\textrm{if}~\low{x} \geq 0 \\
                      & = & [\high{x}^n, \low{x}^n ] ~\textrm{if}~\high{x} < 0\\
                      & = & [0, max\{\low{x}^n, \high{x}^n\} ]~\textrm{otherwise}
  \end{aligned}$
\end{enumerate}
\end{enumerate}
\iffalse

. Algorithm~\ref{alg:precision}
shows the complete description of the bitwidth estimation algorithm applied
at each stage of the DAG computation. We do not show how an expression such
as $x ^ n$, where $n$ is a compile-time constant, is handled in
Algorithm~\ref{alg:precision} for the sake of simplicity. The interval
arithmetic for exponentiation operation, $[\low{x}, \high{x}]^n$ , is defined
as follows.
\begin{eqnarray*}
  [\low{z},\high{z}]  & = & [\low{x}^n, \high{x}^n ] ~\textrm{if}~\low{x} \geq 0 \\
                      & = & [\high{x}^n, \low{x}^n ] ~\textrm{if}~\high{x} < 0\\
                      & = & [0, max\{\low{x}^n, \high{x}^n\} ]~\textrm{otherwise}
\end{eqnarray*}

Our compiler maps simple expressions such as $x*x$ into $x^2$ as this results
in better range estimates. For example, if the range of a signal $x$ is
$[-2, 2]$, then $x*x = [-2, 2]*[-2, 2] = [-4, 4]$, whereas
$x^2 = [-2, 2]^2 = [0, 4]$.

%
 \begin{table}[htb]
     \centering
     \small
     \caption{HCD range analysis and integral bitwidth requirement at various stages.
     \label{tab:hcdbit}}
 \vskip 5pt
 \begin{tabularx}{0.9\linewidth}{lcc}
     \toprule
     Stage & Range & $\alpha$  \\
     \midrule
     Img & $[0,255]$ & $8$ \\
     I$_x$,I$_y$ & $[-85,85]$ & $8$  \\
     I$_{xy}$ & $[-85^2,85^2]$ & $14$  \\
     I$_{xx}$, I$_{yy}$ & $[0, 85^2]$ & $13$  \\
     S$_{xy}$ & $[-9*85^2,9*85^2]$ & $17$ \\
     S$_{xx}$, S$_{yy}$ & $[0, 9*85^2]$ & $16$ \\
     det & -$[-(9*85^2)^2, (9*85^2)^2]$ & $33$  \\
     trace & $[0,2*9*85^2]$ & $17$  \\
     %harris & {\tt [-676650150,676650150]} & 31 & see \\
     harris & $[-1.16*(9*85^2)^2, (9*85^2)^2]$ & $34$ \\
     \bottomrule
 \end{tabularx}
 \end{table}
%
Figure~\ref{fig:hdag} shows the DAG corresponding to the HCD benchmark.
For the sake of simplicity, instead of showing the PolyMage program,
we summarized the computations at each stage in Table~\ref{tab:hcd}.
Table~\ref{tab:hcdbit} summarizes the
ranges and worst case precision requirements of various stages in HCD
as estimated by the range analysis algorithm. It can be noted from the
Table~\ref{tab:hcdbit} that the
bitwidth requirement of $det$ and $Harris$ stages is slightly greater than
the 32 bits required for a
floating-point computation. But the power, area and the delay associated
with fixed point arithmetic at this length could still be better than the
floating-point arithmetic operations.
\fi
%
\iffalse
The range associated
with each pixel of input image is $[0,255]$ as it is an 8-bit image. The
required integral bitwidth $\alpha_{img}$ at this stage is 8. Stages $I_x$
and $I_y$  compute the derivative of the image along $x$ and $y$ axes
respectively. The specific 3x3 stencil operations performed by these stages
can be noted from the Table~\ref{tab:hcd}. The stencil operation here
can be expanded in the form of an expression and the range associated with
it comes out to be $[-85,85]$. Eight integral bits are required to
represent this range.  Stage $I_{xy}$ performs a point-wise computation
using the expression $I_{x,y}(i,j) = I_x(i,j)*I_y(i,j)$. Based on this,
we get the range of the variable $I_{x,y}$ as  $[-85^2, 85^2]$.
Our compiler deduces that the computation at
the stages $I_{xx}$ and $I_{yy}$ is a squaring operation and appropriately
infers the output signal range as $[0, 85^2]$.


Stages $S_{xx}$ , $S_{xy}$ and $S_{yy}$ perform a stencil
operation involving only summation but no division. Expanding the stencil to
an expression form gives us simple addition of neighbouring pixels. The
range we get here for stage $S_{xy}$ is $[-9*85^2,9*85^2]$, and for stages
$S_{xx}$ and $S_{yy}$ is $[0, 9*85^2]$. In a similar fashion, the range
and the associated bitwidths for the stages $det$, $trace$ and $Harris$
can be inferred. It can be noted from the Table~\ref{tab:hcdbit} that the
bitwidth requirement of $det$ and $Harris$ stages is slightly greater than
the 32 bits required for a
floating-point computation. But the power, area and the delay associated
with fixed point arithmetic at this length could still be better than the
floating-point arithmetic operations. Table~\ref{tab:hcdbit} summarizes the
ranges and worst case precision requirements of various stages in HCD.
\fi
%

\subsection{Bitwidth Analysis Compilation Framework}\label{sec:ca}
The interval arithmetic based range analysis algorithm proposed in the
previous section uses the fact that all the pixel signals in each stage of an
image processing DAG are homogeneous in nature and groups them to do a
combined range analysis. However, other analysis techniques such as those
based on affine arithmetic cannot be applied on the DSL level programs in the
same fashion. In this section, we show how interval and affine arithmetic based 
range analysis techniques can be deployed with ease in the PolyMage compilation 
framework.

Recall that the PolyMage-HLS compiler translates a DSL program into C++ code
which the Xilinx Vivado HLS compiler synthesizes into an equivalent circuit
for a target FPGA.  For example, Listing~\ref{lst:sobel} depicts the C++ code
generated by the PolyMage-HLS compiler when Sobel-x filter is applied on an
input image. The generated C++ program can be run in a purely simulation
mode after compilation on any processor by providing test input images as
stimulus. It can be noted from the Listing~\ref{lst:sobel}, that the data type
of the stream, line and window buffers are parameterized by the type
{\tt\bf typ}. It can be a float or any fixed-point data type $(\alpha, \beta)$.
During the hardware synthesis or in the simulation mode, using the C++
polymorphism feature, corresponding libraries for the arithmetic operations
will be invoked based on the operand types.
Now, the parameter {\tt\bf typ} can also be set to an interval type which is
defined in a suitably chosen interval analysis library. If the generated C++
program contains a statement $x=y+z$, then depending on the type of the
variables $x$, $y$ and $z$ (like float, ia-type, aa-type etc.), appropriate
addition operation will be invoked. For example, in order
to perform affine arithmetic analysis on the Sobel-x program, using the
Yet Another Library for Affine Arithmetic (YalAA)~\cite{yalaa}, all we have to
do is to define the parameter {\tt\bf typ} appropriately as depicted in
Listing~\ref{lst:yalaa}.
%
\begin{table}[t]
    \noindent\begin{minipage}[t]{.47\textwidth}
    \begin{lstlisting}[language=C,label={lst:sobel},
    breaklines=true,
    basicstyle=\footnotesize,
    numbers=left, 
    keywordstyle=\sffamily\bfseries\color{green!40!black}, commentstyle=\itshape\color{purple!40!black},
    morekeywords={typ}, identifierstyle=\color{blue},frame=single,%captionpos=b,
        caption=Auto-generated restructured HLS code for Sobel-x.]
    #include <hls_stream.h>
    #include <malloc.h>
    #include <cmath>
    #include <arith.h>
    
    void sobel_x(hls::stream<typ> & img, 
                 hls::stream<typ> & sobel_x_out) 
    {
      const int  _ct0 = (2 + R);
      const int  _ct1 = (2 + C);
      hls::stream<typ> Ix_out_stream;
      hls::stream<typ> img_Iy_stream;
      typ  Ix_img_LBuffer[3][_ct1];
      typ  Ix_img_WBuffer[3][3];
      typ  Ix_img_Coeff[3][3];
    
      /* Code for Sobel-x stage follows. */
    }
    \end{lstlisting}
    \end{minipage}\hfill
      \begin{minipage}[t]{.47\textwidth}
    \begin{lstlisting}[language=C,label={lst:yalaa},breaklines=true,
    basicstyle=\footnotesize\ttfamily,keywordstyle=\sffamily\bfseries\color{green!40!black}, commentstyle=\itshape\color{purple!40!black},
    numbers=left, 
    morekeywords={typ}, identifierstyle=\color{blue}, frame=single,framexbottommargin=100pt,%captionpos=b,
        caption=Type definitions for Affine and Interval Analysis.]
    // Switch for Affine analysis 
    #ifdef AFFINE
    #include <yalaa.hpp>
    typedef yalaa::aff_e_d typ;
    #endif
    // Switch for Interval analysis 
    #ifdef INTERVAL
    #include <Easyval.hpp>
    typedef Easyval typ;
    #endif
    \end{lstlisting}
    \end{minipage}
    \end{table}
%
When we run
the generated C++ program with this data type definition, the value
associated with each pixel in each stage of the pipeline DAG is its affine
signal value which contains the base signal and the coefficients for the noise
variables. From this the range of every pixel can be derived as explained
before. If the data type corresponds to interval arithmetic, then the value
associated with each pixel is an interval. Using this approach, any kind
of interval analysis technique can be deployed in the PolyMage-HLS compiler
easily without re-architecting the analysis backend.

In the next section, we show how interval arithmetic based techniques can
fare really poorly if the benchmarks contain certain kinds of computational
patterns; we use an Optical Flow algorithm as an example. We then  propose our new range analysis technique using SMT solvers.

\iffalse
HAVE TO WORK ON THE NEXT PARA

In the next section, we show that the integral  bitwidth requirements at
various stages  could be smaller than the estimates obtained
through static analysis. This could be due to the nature of the input images
and/or certain correlation between computations on spatially proximal pixels.
 Furthermore, we show how we can use simple binary search to compute the
required fractional bits via program profiling using an application-specific
error metric. In these estimations of integral and fractional bitwidth, we
can also exploit the fact that many image processing applications are
resilient to small arithmetic overflow/precision errors, to arrive at power
and area-efficient hardware designs by using practical estimates for data
range and precision.
\fi

\input{files/smt}

\subsection{Profile-Driven Analysis}
\label{sec:profile}
Profile-driven analysis can be used to accomplish two tasks. First, we can obtain
lower bounds on the bitwidth estimates, which can be compared with the estimates
obtained using static analysis. Second, depending on the application, these 
estimates
can be used in the actual system design instead of the conservative 
estimates obtained through static analysis techniques. However, the
bitwidth  requirements estimated at each stage using profiling naturally 
depend on the sample input images. Based on the analysis done by Torralba et 
al. \cite{torralba2003statistics}, we hypothesize that the
images taken from a certain domain, like for example {\it nature}, has
similar properties, and hence the bitwidth estimates can be carried over to
other images drawn from the same domain.

%
\subsubsection{Integral Bits}
The number of integral bits required at a stage $i$ denoted as $\alpha_i$  can
be obtained by running the input PolyMage program on a sample  distribution of
input images. Let $\alpha_i^s$ be the maximum number of bits  required by stage
$i$ to represent a pixel from an image sample $s$. Then  the average number of
bits $\alpha_i^{avgP}$ required based on a sample set  $S$ is $\sum_{s\in S}
\alpha_i^s/|S|$. Similarly, the worst-case number of  bits $\alpha_i^{maxP}$
required is $max_{s\in S} \alpha_i^s$. We can either  use $\alpha_i^{avgP}$ or
$\alpha_i^{maxP}$ as estimates for $\alpha_i$. Even if the estimate does not
suit certain images, in many application  contexts, using saturation mode
arithmetic results in satisfying the desired  output quality metric. Let
$\alpha_i^{IA}$ and $\alpha^{\smtra}$ be the integral bitwidth  estimates
obtained for stage $i$ through interval analysis and \smtra\ analysis
respectively. For the benchmarks we have considered, affine analysis show some
improvements in the range estimates, but it amounts to same bitwidth requirement
as with interval analysis. Hence,  throughout the rest of the paper, we consider
only interval analysis.

For our experimentation, we used a subset of 200 randomly chosen images from
the Oxford Buildings dataset~\cite{oxfordimages} consisting of 5062 images.
The set of 200 images is partitioned into two equal halves: training and
test sets. The training set is used to obtain estimates of integral
bitwidths at various stages through profiling. The test set is used to
evaluate the effectiveness of the bitwidth estimates obtained for quality
and power. Figure~\ref{fig:hs} shows the average cumulative distribution of
the bitwidth required by the integral part of the pixels in stages $I_x$
and $I_{xy}$  of the HCD benchmark on the training data set.
\iffalse
The x-axis of the graphs represent the bitwidth requirement of the integral
part, and y-axis represents the percentage of pixels, averaged across test
images, that can be represented within a given bitwidth.
\fi
For example, from Figure~\ref{fig:hs}, we can infer that in stage $I_x$,
95\% of the pixels require less than 5 bits, and all pixels (100\%) can be represented
using 8 bits.
\iffalse
Since
stages $I_x$ and $I_y$ are of similar computational nature, we plot the
histogram for only $I_x$.  Similarly, among $I_{xx}$, $I_{xy}$ and $I_{yy}$,
we plot for $I_{xy}$ in Figure~\ref{fig:hs2}, and from stages $S_{xx}$,
$S_{xy}$ and $S_{yy}$, we plot for $S_{xy}$ in Figure~\ref{fig:hs3}.
Figures~\ref{fig:hs4},~\ref{fig:hs5} and~\ref{fig:hs6} correspond to {\it
det}, {\it trace} and {\it Harris} stages respectively.

Table~\ref{tab:bitTableHCD},~\ref{tab:bitTableUSM_DUS} shows the bitwidth estimates obtained from
static and profile-driven analyses.
\fi
Table~\ref{tab:bitTableHCD} shows the bitwidth estimates obtained from
static and profile-driven analyses for the HCD benchmark.
%
\begin{table*}[h!]
    \footnotesize
    \caption{Comparison of integral bitwidth estimates using interval, \smtra, 
    and profile-guided analyses for HCD. Fractional bitwidth estimates are also provided in the last row.}
    \vskip 5pt
    \label{tab:bitTableHCD}
\centering
    %\resizebox{0.5*\textwidth}{!}{%
        \begin{tabular}{c | c c c c c c c c c}
        \toprule
        & &&&&HCD&&&&\\
        Stage&Img&I$_x$,I$_y$&I$_{xx}$,I$_{yy}$&I$_{xy}$&S$_{xy}$&S$_{xx}$, S$_{yy}$&det&trace&harris\\
        \midrule
        $\alpha^{\smtra}$ &          8&8&13&14&17&16&33&17&\bf{33}\\
        $\alpha^{IA}$ & 8&8&13&14&17&16&33&17&34\\
        \midrule
        $\alpha^{maxP}$& 8&8&13&14&17&16&30&17&29\\
        $\alpha^{avgP}$& 8&8&13&14&17&16&29&17&29\\
        \midrule
        $\beta$ & 8&5&4&4&3&3&1&1&1       \\
        \bottomrule
        \end{tabular}
       % }%
\end{table*}
%

%
As can be noted from
Table~\ref{tab:bitTableHCD}, the bitwidth estimates from $\alpha^{avgP}$
and $\alpha^{maxP}$  measures are the same for all stages
except for the {\it det} stage.
The estimates from the static analysis techniques match the profile estimates 
except for the {\it det}, {\it trace} and {\it harris} stages. In general, we
expect the profile estimates to be better for stages that occur deeper in
the pipeline. Unlike Optical Flow benchmark, for HCD, \smtra\ analysis 
performs no better than interval analysis except for a single bit 
improvement in stage {\it Harris}. Again, we note that the profile estimates 
also indicate the limit to which the static analysis techniques can be 
improved by using more powerful approaches. Profile information can be 
easily
obtained by executing the HLS C++ program directly without the need for a
heavy weight circuit simulation.

In the next section, we propose a simple and practical greedy search 
algorithm to estimate the number of fractional bits at each stage of the DAG 
while respecting an application specific quality constraint.
%
\iffalse
\begin{figure}[hb]
%\captionsetup[subfigure]{labelfont=bf,textfont=normalfont}
\centering
\resizebox{\columnwidth}{!}{%
  \harrisHist
  }%
    \vskip 5pt
\caption{Cumulative distribution of pixels with respect to maximum integral bitwidth length at
 stages $I_x$ and $I_{xy}$ of the HCD benchmark.}
\label{fig:hs}
\end{figure}
\fi
% Separate file for SMT section

\subsubsection{Fractional Bits ($\beta$) Analysis}\label{sec:precision}
The number of fractional bits $\beta_i$ required at a stage $i$ depends on the
application and cannot be estimated in an application independent manner 
similar to the integral bitwidth analysis. Estimating the optimal number of
fractional bits at each stage for a given application metric turns out to be a
non-convex optimization problem in most cases and hence we propose a simple
heuristic search technique that requires a very small number of profile 
passes.

In the profiling technique, we fix the number of integral bits required at 
each stage based on static or profile-driven analysis and increase the 
precision
$\beta$ uniformly across all stages. For each value $\beta$, we estimate
the application-specific error metric. For the HCD benchmark, the error
metric is the percentage of misclassified corners when compared to a design
that uses sufficiently long integral and fractional bits. We can reach an
optimal $\beta$ for a given error tolerance via binary search. Then we make
a single pass on the stages of the DAG in  reverse topologically sorted 
order.
At each stage $I$, we do a binary search on the number of fractional bits
required, $\beta_I$, starting from the initial estimate $\beta$ while
retaining the application specific quality requirement. The last row 
of the Table~\ref{tab:bitTableHCD} shows the fractional bits estimated
at each stage of the HCD benchmark. Note that the later stages of the DAG 
require fewer bits than those stages which occur earlier in the DAG. 
This is due to the fact that errors in earlier stages will have a
greater impact as they get propagated to the downstream stages. Further,
our greedy algorithm is optimizing the bitwidths by considering the 
stages in the reverse topologically sorted order. 
\input{files/flow}
\subsection{Summary of Bitwidth Analysis Framework}
Figure~\ref{fig:flow} summarizes the proposed bitwidth analysis framework. 
We can use the PolyMage-HLS compilation framework first to do a range analysis and 
estimate the integral bitwidths; then use the greedy heuristic to estimate the 
fractional bits required at various stages. For range analysis, we can use one of interval, 
\smtra\ and profile analysis techniques. For interval analysis, the compiler generates
HLS code where the data types of the variables at various stages of the DAG are intervals.
Then the bitwidth estimates are obtained using the intervals obtained by running the HLS 
code. For profile analysis, the compiler generates HLS code wherein the data types of
the variables are of fixed point type with sufficiently large integral and fractional
bitwidths. Then HLS code is run on a sample distribution of input images to arrive at 
integral bitwidth estimates.  For \smtra\ analysis, the compiler generates a 
constraint system which is solved by an SMT solver, such as Z3, to arrive at 
range estimates. 

\iffalse
\begin{table*}[h!]
    \footnotesize
    \caption{Comparison of integral bitwidth estimates using interval, \smtra, 
    and profile-guided analyses for USM and DUS. Fractional bitwidth estimates are also provided in the last row.}
    \vskip 5pt
    \label{tab:bitTableUSM_DUS}
\centering
    %\resizebox{\linewidth}{!}{%
        \begin{tabular}{c | c c c c c | c c c c c }
        \toprule
        &&&USM&& &&&DUS&&\\
        Stage&Img&blur$_x$&blur$_y$&sharpen&mask&Img&D$_x$&D$_y$&U$_x$&U$_y$\\
        \midrule
        $\alpha^{Z3RA}$ &8&8&8&10&9 &8&8&8&8&8\\
        $\alpha^{IA}$  &8&8&8&10&9 &8&8&8&8&8\\
        \midrule
        $\alpha^{maxP}$ &8&8&8&10&9 &8&8&8&8&8\\
        $\alpha^{avgP}$ &8&8&8&10&9 &8&8&8&8&8\\
        \midrule
        $\beta$  &0&2&3&4&4  &0&3&6&8&10\\
        \bottomrule
        \end{tabular}
        %}%
\end{table*}
\fi


==> files/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
The input, output and intermediate values generated in many image processing
applications have a limited range. Furthermore, these  applications are
resilient to errors arising from factors such as limited  precision
representation, inaccurate computations, and other potential noise  sources. In
this work, we exploited these properties to generate power and  area-efficient
hardware designs for a given image processing pipeline by  using custom
fixed-point data types at various stages. We showed that domain-specific 
languages facilitate the application of interval and affine arithmetic 
analyses on larger benchmarks with ease. Further, we proposed a new 
range analysis technique using SMT solvers, which overcomes the inherent 
limitations in conventional interval/affine arithmetic techniques, when 
applied to iterative algorithms. The proposed SMT solver based range 
analysis technique also uses the DSL specification of the program to reduce 
the number of constraints and variables in the constraint system, thereby 
making it a feasible technique to adopt in practice. Then, we compared the 
effectiveness of the static analysis techniques against a profile-driven 
approach that automatically takes into account properties of input image 
distribution and any correlation between computations on spatially proximal 
pixels. In addition, the analysis revealed the limit of possible improvement 
for any static analysis technique for integral bitwidth estimation.  
Finally, to estimate the number of fractional bits, we used uniform 
bitwidths across all the stages of the pipeline, and then used a simple 
greedy search to arrive at a suitable bitwidth at each stage while 
satisfying an application-specific quality criterion. Overall, the results 
effectively demonstrate how information exposed through a high-level DSL 
approach could be exploited in practical fixed-point data type analysis 
techniques and to perform detailed impact studies on much larger image 
processing pipelines than previously studied.
%
% We use uniform fractional bitwidth across all stages of computation.
%
\iffalse
theoretical improvements we can

Our bitwidth estimation algorithms rely

In this paper, we proposed an interval arithmetic-based integral bitwidth
analysis algorithm for image processing pipelines. The algorithm is simple
and nicely fits into the data flow analysis framework used in compilers.
Then, we compared the effectiveness of the static analysis algorithm against
a profile-driven approach that automatically takes into account
properties of input image distribution and any correlation between
computations on spatially proximal pixels.  For precision analysis, to
estimate fractional bits, we use uniform bitwidths across all the stages of
the pipeline, and then use a simple search to arrive at a suitable bitwidth
that satisfies an application-specific quality criterion.  In conclusion,
our experimental evaluation demonstrates that by using variable bitwidth
fixed-point numbers at various stages of an image processing pipeline, get
substantial power and area savings can be obtained without a loss in desired
quality.
\fi
%
\iffalse In this paper, we proposed an automatic precision analysis algorithm
which in a very simple and efficient manner  leverages the power and area
savings, as demonstrated on various image processing benchmarks. The algorithm
nicely fits into the data flow analysis framework used in compilers. We
developed an interval arithmetic based static algorithm for range analysis.
Then, we compared the effectiveness of the static analysis algorithm against  a
profile-driven approach that automatically takes into account properties of
input image distribution and any correlation between computations on spatially
proximal pixels and showed that we were able to perform at par with static
precision using lesser area and power. For precision analysis, to estimate
fractional bits, we proposed a profiling based approach that uses uniform bit-
widths across all the stages of  the pipeline, and then use a simple search to
arrive at a suitable bitwidth  that satisfies an application-specific quality
criterion, which we carefully arrived at to compare the performance of our
algorithm.  Finally, we  demonstrate that by using the precision obtained using
our analysis, we we can get substantial power and area savings without a loss in
desired quality.
\fi



==> files/experiments.tex <==
\section{Experimental Results}\label{sec:experiments}
In this section, we present a detailed area, power and throughput analysis when
variable fixed-point data types are used as against floating-point by 
considering the following four benchmarks: Harris Corner Detection, Unsharp
Mask, Down and Up Sampling, and Optical Flow. Tables~\ref{tab:ofrange},
~\ref{tab:bitTableHCD},~\ref{tab:bitTableUSM} and~\ref{tab:bitTableDUS} show the integral bitwidth 
estimates obtained through interval analysis ($\alpha^{IA}$), \smtra\ analysis
($\alpha^{\smtra}$) and profile analysis ($\alpha^{maxP}$ and $\alpha^{avgP}$); 
and the average fractional bitwidth estimate ($\beta$) obtained through greedy 
heuristic search algorithm. Table~\ref{tab:Allresults} compares the performance
of each benchmark using {\it float} data type and bitwidth estimates obtained 
from different approaches. In these tables, the {\it Quality} column  
corresponds to an application specific quality metric; the {\it Power} 
column gives the power when the design operates at a speed specified in the
adjacent {\it Clk Period} column; {\it latency} columns provide the number 
of
clock cycles required to process an HD image; the next four columns (BRAM,
DSP, FF, LUT, \%slices) summarize area usage; the {\it Min Clk Period}
column gives the maximum frequency of operation for circuit; and the next 
two columns give the throughput and power consumed at the maximum frequency
of operation. Figure~\ref{fig:powersplit} gives the split of power usage by
various components of an FPGA. Unlike the Optical Flow benchmark, the integral 
bitwidth estimates for the benchmarks HCD, USM and DUS using interval and 
\smtra\ analysis techniques is the same. So we do not provide separate area, 
power and throughput analysis for these benchmarks.

We used the Xilinx Zedboard consisting of Zynq-XC7Z020 FPGA device and 
Xilinx Vivado Design Suite 2017.2 version to conduct our experiments. The 
HLS design generated by our PolyMage DSL compiler is synthesized by the 
Vivado HLS compiler. All characteristics are reported post Place and Route.  
We ran C-RTL
co-simulations to generate switching activity (SAIF) file for reporting 
detailed power consumption across the design. 



%We use the same dataset for all the benchmarks for profiling them.
% see here if you want to keep this figure
\begin{table*}[t]
    \footnotesize
    \caption{Power, area and throughput analysis for HCD, DUS, USM and OF benchmarks using float and integral bitwidth estimates obtained using
    static and profile-driven analyses. Fractional bitwidths are determined based on the greedy heuristic search approach.}
    \vskip 5pt
    \label{tab:Allresults}
    \centering
    \Ress
\end{table*}

\subsection{Harris Corner Detection}
Table~\ref{tab:bitTableHCD} summarizes the integral and fractional bitwidth estimates 
obtained at each stage of the HCD benchmark through various analysis techniques.
The results in this table are commented upon in Sections~\ref{sec:profile} 
and~\ref{sec:precision}. Figure~\ref{fig:uniformbeta} shows the average percentage of 
pixels correctly 
classified by the HCD benchmark on the test image set by varying the 
fractional bits uniformly across all the stages while fixing the integral 
bitwidth estimates obtained via profiling ($\alpha_i^{avgP}$). It also 
contains estimates of power consumption with varying fractional bits for the 
Xilinx ZED FPGA board.
It can be noted from the graph that the fractional bits do not affect the 
accuracy of corner classification, and we thus get more than 99\% accuracy 
even with zero fractional bits. From this graph, we infer that one can 
obtain close to 100\% accuracy by using 8 fractional bits uniformly across 
all the stages. We then make a backward pass on the stages of the
HCD benchmark to drop the fractional bits further without any significant loss
in accuracy and the row corresponding to $\beta$ in 
Table~\ref{tab:bitTableHCD} shows the final fractional bitwidths. Due to space
constraint, we do not provide a graph such as Figure~\ref{fig:uniformbeta} for
the rest of the benchmarks. We can notice from Table~\ref{tab:Allresults} that by 
using bitwidth estimates from interval analysis, we obtain 99.999\% accuracy with
a power consumption of 0.263~W. The power savings are 
3.8$\times$ lower when compared with the floating-point design and 4\% more when 
compared with the profile-estimate based design. The savings
on the percentage of FPGA slices used is around 6.2$\times$. From the last 
3 columns of the table, we can notice that the fixed-point designs can operate
at a higher frequency achieving better throughput while consuming lesser power. 

Figure~\ref{fig:powersplit} shows the detailed power analysis for floating-point and fixed-point design. It shows only the significant components of the dynamic power consumed, and in all the designs, the static power consumption is around 0.122~W.
\begin{figure}[!htb]
    \centering
    \begin{minipage}[t]{0.45\textwidth}
        \centering
\resizebox{\linewidth}{!}{
        \harrisProfPower
        }
        \caption{Error and power variation for the HCD benchmark by fixing the number of integral bits to profile estimated values $\alpha_i^{avgP}$ and varying $\beta$ uniformly across all the stages.}
        \label{fig:uniformbeta}
    \end{minipage}%
    \hfill
    \begin{minipage}[t]{0.45\textwidth}
        \centering
\resizebox{\linewidth}{!}{
        \includegraphics{./graphs/hcd_power_graph}
        }
        \caption{Power consumption by individual components on FPGA for HCD.\label{fig:powersplit}}
    \end{minipage}
\end{figure}

\iffalse
\begin{figure}[htbp]
\centering
\resizebox{0.8\linewidth}{!}{
                \harrisProfPower
            \label{fig:haProf}
            }
\vskip 5pt
\caption{Error and power variation for the HCD benchmark by fixing the number of
 integral bits to profile estimated values $\alpha_i^{avg}$ and varying 
 $\beta$ uniformly across all the stages.}
 \label{fig:uniformbeta}
\end{figure}
\fi


\begin{figure*}[!htb]
    \begin{minipage}[t]{0.49\linewidth}
        \centering
    \resizebox{0.95\linewidth}{!}{
        \usmDag
    }
    \caption{Pipeline DAG structure for USM benchmark.}
    \label{fig:USMdag}
    \end{minipage}
    \begin{minipage}[t]{0.49\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c | c c c c c }
        \toprule
        Stage&Img&blur$_x$&blur$_y$&sharpen&mask\\
        \midrule
        $\alpha^{Z3RA}$ &8&8&8&10&9 \\
        $\alpha^{IA}$  &8&8&8&10&9 \\
        \midrule
        $\alpha^{maxP}$ &8&8&8&10&9 \\
        $\alpha^{avgP}$ &8&8&8&10&9 \\
        \midrule
        $\beta$  &0&2&3&4&4  \\
        \bottomrule
        \end{tabular}
        }%
        \captionof{table}{Comparison of integral bitwidth estimates using interval, \smtra, and profile-guided analyses for USM. Fractional bitwidth estimates are also provided in the last row.}
        \label{tab:bitTableUSM}
\end{minipage}
\end{figure*}


\subsection{Unsharp Mask (USM)}
The Unsharp Mask (USM) benchmark sharpens an input image and its computational
DAG is provided in Figure~\ref{fig:USMdag}. The input image is blurred across 
x-axis and y-axis by the stencil stages {\it blurx} and 
{\it blury} successively. Then it passes through 
the {\it sharpen} stage, which is a point-wise computation.  Finally, the 
{\it masked} stage compares each pixel from the output of the {\it sharpen} 
stage with a threshold value. Depending on whether the pixel value is less 
than threshold, the corresponding pixel from either the original input image 
or the sharpened image is chosen for output. We highlight an important 
observation here: even if we make an error in computing a pixel value from 
the {\it sharpen} stage, as long as it is less than the threshold, the right 
output pixel is chosen. Based on this observation, we define an error metric 
that is the fraction of pixels that were misclassified in the {\it masked}  
stage due to variable width fixed-point representation as against 
floating-point representation. We define a second quality metric that is the 
root mean squared error between correctly classified pixel values and their 
floating-point counterparts.

Table~\ref{tab:bitTableUSM} shows the integral and fractional bitwidths
required at various stages of the USM benchmark obtained from static (interval
and \smtra) and profile analyses. It can be noted that the estimates obtained by
the static and profile analyses are the same. Table~\ref{tab:Allresults} shows
that there is a factor of 1.6$\times$ improvement in power when compared to the
floating-point design with negligible root mean squared error and classification
error. With respect to the number of FPGA slices used, there is a factor of
2.6$\times$ improvement. Table~\ref{tab:Allresults} also shows the maximum
frequency of operation for each of the designs, the throughput at that level and
power consumption. From the last 3 columns of the table, we can infer that by
operating the fixed-point design at a higher frequency, 6\% increase in
throughput can be achieved while consuming 1.7x lower power.

\begin{figure*}[!htb]
    \begin{minipage}[t]{0.49\linewidth}
    \centering
    \resizebox{0.95\linewidth}{!}{
            \dusDag
    }
    \caption{Pipeline DAG structure for DUS benchmark.}
    \label{fig:DUSdag}
    \end{minipage}
    \begin{minipage}[t]{0.49\linewidth}
    \centering
    \resizebox{0.8\linewidth}{!}{%
        \begin{tabular}{c | c c c c c }
        \toprule
        Stage&Img&D$_x$&D$_y$&U$_x$&U$_y$\\
        \midrule
        $\alpha^{Z3RA}$ &8&8&8&8&8\\
        $\alpha^{IA}$   &8&8&8&8&8\\
        \midrule
        $\alpha^{maxP}$  &8&8&8&8&8\\
        $\alpha^{avgP}$  &8&8&8&8&8\\
        \midrule
        $\beta$    &0&3&6&8&10\\
        \bottomrule
        \end{tabular}
    }
    \captionof{table}{Comparison of integral bitwidth estimates using interval, \smtra, and profile-guided analyses for DUS. Fractional bitwidth estimates are also provided in the last row.}
    \label{tab:bitTableDUS}
    \end{minipage}
\end{figure*}

\subsection{Down and Up Sampling (DUS)}
Down and Up Sampling (DUS) benchmark has a linear DAG structure as shown in Figure~\ref{fig:DUSdag}. The image is first 
downsampled along the $x$-axis in stage D$_x$ and is further downsampled along the $y$-axis in stage D$_y$.
It  is then upsampled again along the $x$ and $y$ axes in the stages $U_x$ and $U_y$ 
respectively. For the sake of conciseness, we avoid including the DUS 
PolyMage code. All four stages comprise stencil computations.

The integral bitwidths estimated by both the interval and \smtra\ analyses is
equal to 8 at all the stages of DUS. We use the same set of training images as
that of HCD benchmark for estimating the integral and fractional bitwidths via
profiling.  The profile estimates yielded the same integral bitwidth requirement
of 8 at all the stages. We use Peak Signal to Noise Ratio (PSNR) as a quality
metric where the reference image is obtained by using a sufficiently wide data
type. We set the required PSNR to infinity and the resulting fractional
bitwidths determined by our greedy precision analyzer is shown in the last row
of the Table~\ref{tab:bitTableDUS}. Table~\ref{tab:Allresults} shows that there
is a factor of 1.7$\times$ reduction in power using tuned fixed-point data types
when compared with using floating-point data type without loss of any accuracy.
With respect to area, there is a 4$\times$ improvement in terms of number of
slices used.   Also, the fixed-point designs use no DSP blocks at all when
compared with floating-point design which uses 54 DSPs. At the peak possible
frequency of operation, fixed-point design achieves 13.6\% increase in
throughput while consuming 1.6x lesser power.


\subsection{Optical Flow (OF)} 
The Optical Flow (OF) benchmark computes the velocity of individual pixels 
from an image frame and its time-shifted version. Our implementation is 
based on  the Horn-Schunck algorithm \cite{horn1981determining} and consists 
of 30 stages.  The first 10 stages are pre-processing stages and the last 20 
stages are obtained by repeating a set of five stages for four times.  The 
accuracy of motion estimation can be improved by repeating  the 5-stage set 
more times.  Optical flow is a heavily used image processing algorithm in 
many computer vision applications.
There have been many efforts in the past to implement optical flow on 
FPGAs~\cite{JavierTCSVT'06,AlanISSC'10,EnZhuTCSVT'16} for power and 
performance benefits.

Table~\ref{tab:ofrange} shows the estimated integral bitwidths required 
at various stages of the Optical Flow benchmark. We notice that for stages 
deeper in the pipeline, the difference between estimates obtained via interval  
analysis and profiling are substantial. The profile estimates are obtained 
from a training data set and for testing purpose, we use RubberWhale and 
Dimetrodon image sequences from the Middlebury dataset~\cite{MBuryDataSet}.  
Section~\ref{sec:smt} provides a detailed discussion on this and shows how 
the \smtra\ analysis can overcome the inadequacies of the interval arithmetic
based analyses techniques and gives estimates which almost match profile estimates.
For computing the accuracy, we use the Average Angular Error (AAE) metric as 
discussed in \cite{Fleet:1990},\cite{Otte:1994}. The reference motion 
vectors are obtained by using sufficiently wide fixed-point data types at 
all stages. 

It can be noticed from Table~\ref{tab:Allresults} that by  using bitwidth
estimates from Z3RA analysis, we obtain similar accuracy as  profile-driven
analysis with a power consumption of 0.328~W. The power savings are  1.9$\times$
lower when compared with the floating-point design and 5.4\% more when  compared
with the profile-estimate based design. The savings on the percentage of FPGA
slices used is around 2.5$\times$.  From the last 3 columns of the table, we can
notice that the Z3RA fixed-point design can operate at a higher frequency
achieving 25\% more throughput than the floating point design while consuming
lesser power.

%
\iffalse
\begin{table*}[htbp]
    \footnotesize
    \caption{Metrics for the OF benchmark using float, and using bitwidths estimated using static analysis and profiling techniques.}
    \vskip 5pt
    \label{tab:OFresults}
\centering
    \ofRes
\end{table*}
%
\begin{table*}[htbp]
    \footnotesize
    \caption{Metrics for USM benchmark using float, and using bitwidths estimated using static analysis and profiling techniques. }
    \vskip 5pt
    \label{tab:USMresults}
\centering
    \usmRes
\end{table*}
%
\begin{table*}[htbp]
    \footnotesize
    \caption{Metrics for DUS using float, and using bitwidths estimated using static analysis and profiling techniques. }
    \vskip 5pt
    \label{tab:DUSresults}
\centering
    \dusRes
\end{table*}
\fi
%
\iffalse
\begin{table}[tb]
\footnotesize
    \centering
    \caption{Comparison of bitwidth estimates using profiling technique and static analysis for the HCD benchmark.
    \label{tab:hcdintegral}}
\vskip 5pt
\begin{tabularx}{0.8\linewidth}{l|c@{~~~~~~~~~~~}c@{~~~~~~~~~}c@{~~~~~~~~~}|c@{~~~~~~~~~~~}}
    \toprule
    Stage & $\alpha^{sa}$ & $\alpha^{max}$ &  $\alpha^{avg}$ & $\beta^{avg}$   \\
    \midrule
    Img                  & 8  & 8  & 8  & 8\\
    I$_x$,I$_y$          & 8  & 8  & 8  & 5\\
    I$_{xx}$,I$_{yy}$    & 13 & 13 & 13 & 4\\
    I$_{xy}$             & 14 & 14 & 14 & 4\\
    S$_{xy}$             & 17 & 17 & 17 & 3\\
    S$_{xx}$, S$_{yy}$   & 16 & 16 & 16 & 3\\
    det                  & 33 & 30 & 29 & 1\\
    trace                & 17 & 17 & 17 & 1\\
    harris               & 34 & 29 & 29 & 1\\
    \bottomrule
\end{tabularx}
\end{table}
%
\begin{figure*}[htbp]
\centering
    \usmHist
    \vskip 5pt
\caption{Cumulative distribution of pixels with respect to maximum integral bitwidth length at various stages of the USM.}
\label{fig:usm}
\end{figure*}
%% TABLES
\begin{table}[tb]
\footnotesize
    \centering
    \caption{Comparison of bitwidth estimates using profiling technique and static analysis for the USM benchmark.
    \label{tab:usmintegral}}
\vskip 5pt
\begin{tabularx}{0.87\linewidth}{l|c@{~~~~~~~~~~~}c@{~~~~~~~~~~~}c@{~~~~~~~~~~~}|c@{~~~~~}}
    \toprule
    Stage & $\alpha^{sa}$ & $\alpha^{max}$ &  $\alpha^{avg}$ & $\beta^{avg}$   \\
    \midrule
    img                                                       & 8  & 8  & 8  & 0\\
    blur$_x$                                                  & 8  & 8  & 8  & 2\\
    blur$_y$                                                  & 8  & 8  & 8  & 3\\
    sharpen                                                   & 10 & 10 & 10 & 4\\
    mask                                                      & 9  & 9  & 9  & 4\\
    \bottomrule
\end{tabularx}
\end{table}
\begin{table}[!htb]
\footnotesize
    \centering
    \caption{Comparison of bitwidth estimates using profiling technique and static analysis for the DUS benchmark.
    \label{tab:dusintegral}}
\vskip 5pt
\begin{tabularx}{0.80\linewidth}{l|c@{~~~~~~~~~~~}c@{~~~~~~~~~~~}c@{~~~~~~~~~~~}|c@{~~~~~~~}}
    \toprule
    Stage & $\alpha^{sa}$ & $\alpha^{max}$ &  $\alpha^{avg}$ & $\beta^{avg}$     \\
    \midrule
    img                                                         & 8 & 8 & 8 & 0  \\
    D$_x$                                                       & 8 & 8 & 8 & 3  \\
    D$_y$                                                       & 8 & 8 & 8 & 6  \\
    U$_x$                                                       & 8 & 8 & 8 & 8  \\
    U$_y$                                                       & 8 & 8 & 8 & 10 \\
    \bottomrule
\end{tabularx}
\end{table}
%
\fi
%
\iffalse
\begin{figure*}[htbp]
\centering
    \subfloat[Throughput]{
        \includegraphics[width=0.40\linewidth]{graphs/throughput}
    }
     \subfloat[Power]{
        \includegraphics[width=0.40\linewidth]{graphs/power}
    }
    \vskip 5pt
    \caption{Throughput and respective power obtained with various FPGA design benchmarks\label{fig:throughput}}
\end{figure*}
%
\begin{figure}[t]
    \centering
  \resizebox{0.8\columnwidth}{!}{%}{
    \dusDag
   }
\vskip 5pt
\caption{Pipeline DAG structure for DUS benchmark.} \label{fig:DUSdag}
\end{figure}
%

\iffalse
\begin{figure}[htbp]
\centering
\resizebox{0.8\linewidth}{!}{
            %\subfloat[HCD]{
            \harrisProfPower
            \label{fig:haProf}
            %}
            }
            \iffalse
            \subfloat[USM]{
                \usmProfPower
            \label{fig:usmProf}
            } \\
            \subfloat[DUS] {
                \dusProfPower
            \label{fig:dusProf}
            }
            \subfloat[OF]{
                \ofProfPower
            \label{fig:ofProf}
            }
            \fi
\vskip 5pt
\caption{Error and power variation for the HCD benchmark by fixing the number of
 integral bits to profile estimated values $\alpha_i^{avg}$ and varying
 $\beta$ uniformly across all the stages.}
 \label{fig:uniformbeta}
\end{figure}
%
\fi
\begin{figure}%[htbp]
\centering
\resizebox{0.8\linewidth}{!}{
            %\subfloat[HCD]{
            \includegraphics{./graphs/hcd_power_graph}
            %}
            \iffalse
            \subfloat[USM]{\includegraphics{./graphs/usm_power_graph}
            \label{fig:usmsplit}
            }\\
            \subfloat[DUS]{\includegraphics{./graphs/dus_power_graph}
            \label{fig:dussplit}
            }
            \subfloat[OF]{\includegraphics{./graphs/of_power_graph}
            \label{fig:ofsplit}
            }
            \fi
            }
            \vskip 5pt
            \caption{Power consumption by individual components on FPGA for HCD.\label{fig:powersplit}}
\end{figure}
\fi

\iffalse
\begin{figure}%[htbp]
    \centering
    \resizebox{0.8\linewidth}{!}{
                \subfloat[HCD]{
                \includegraphics{./graphs/hcd_power_graph}
                }
            %    \iffalse
                \subfloat[USM]{\includegraphics{./graphs/usm_power_graph}
                \label{fig:usmsplit}
                }\\
                \subfloat[DUS]{\includegraphics{./graphs/dus_power_graph}
                \label{fig:dussplit}
                }
                \subfloat[OF]{\includegraphics{./graphs/of_power_graph}
                \label{fig:ofsplit}
                }
             %   \fi
                }
                \vskip 5pt
                \caption{Power consumption by individual components on FPGA for HCD.\label{fig:powersplit}}
\end{figure}
\fi 



==> files/general-framework-smt.tex <==
\section{Framework}
The polymage code is parsed into an intermediate json representation which contains complete information about the image processing pipeline represented in a DAG form. This IR is particularly useful as it provides modularity and makes addition of more analysis backends possible in the future. The json structure for point-wise and stencil computations is shown in figure ?. The whole image processing DAG can be expressed using this json structure.

From the json representation, a python code is generated which uses the Z3 python API for solving the per-stage bitwidth. 
(I have a doubt on how to justify the the theory we use for Z3. I use theory of Reals. Although i have ran using Bit-Vectors as well which results in unknown solution and sometimes gives an error also for HCD particularly.. Well, as of now i am keeping the theory as an input parameter to the framework).

(Writing about the structure of our framework)

Our Z3 analysis framework is written with parameterised functions for point-wise and stencil computations which makes the code-generation from json straight forward. For each stage the parameters are extracted and the function is called with those parameters. For each stage, there is an option of breaking the correlations and make the output variables fundamental. This is done to deal with complex dags and to make the framework scalable. Figure ? shows the call structure for point-wise and stencil stages. 
%For stencil stages the required parameters are ... and the function ___ returns the following ... For point-wise stage the required parameters are ... and the function ___ returns the following ...

(Next file is running-example-smt.tex)

==> files/introduction.tex <==
\section{Introduction}
Field-Programmable Gate Arrays (FPGAs) are suitable for accelerating
computations from several domains such as image processing, computer vision, 
and digital signal processing. When a lower or customized precision is 
desired,  FPGAs are often expected to perform better than accelerators such 
as GPUs with respect to performance delivered per unit of energy consumed.  
When an image processing pipeline such
as Harris Corner Detection (HCD) (cf. Figure~\ref{fig:hdag} and Table~\ref{tab:hcd}),
is implemented on a CPU or a GPU, a programmer is bound to choose a pre-defined
data type such as {\tt float}, {\tt int}, or {\tt short} owing to the underlying
architectural constraints. In order to avoid arithmetic overflows, the
data types have to be chosen conservatively through over-estimation. This 
leads to a wastage of memory, and hence memory bandwidth, at all levels of 
the hierarchy; furthermore, additional energy is consumed both due to data 
transfer and the higher precision in which the arithmetic is performed.  On 
the other hand, on FPGAs, it is possible to use variable length
fixed-point data types to represent the data produced and consumed at various
stages of an image processing pipeline. This saves chip area and the power
consumed by the hardware design due to the reduced precision
and internal routing logic. The other natural outcome is a better 
utilization of available on-chip memory resources.

Although, FPGAs fare extremely well on the performance per watt metric, 
their programmability has been a major hindrance in adoption. The reliance 
on hardware description languages (HDLs) such as Verilog and VHDL makes it 
extremely cumbersome for a wider programmer audience. High-Level Synthesis 
(HLS) tools, which map C, C++ code into equivalent hardware designs by 
generating HDL code automatically, have thus gained significant attention in 
the past decade. The quality of designs generated by a HLS compiler often 
depend on the analysis techniques employed. Many times programmers put in 
substantial effort to drive a HLS tool to generate a hardware design of 
their choice using suitable pragma annotations or code rewriting. There have 
been efforts to further raise the level of abstraction --- from using 
imperative languages such as C, C++ to domain-specific languages (DSLs) --- 
giving rise to the term, ultra high-level synthesis; Bacon et 
al.~\cite{bacon13acm} provide a comprehensive survey.  DSLs not only
improve programmer productivity but also exploit the richer information  
from the underlying algorithm. This facilitates compilers to generate better 
code or hardware designs using relatively simple program analysis 
techniques.

\subsection{DSLs for Image Processing Pipelines} An image processing 
pipeline can be viewed as a directed acyclic graph (DAG) of computational 
stages. Each stage transforms an
input image form into an output image form to be consumed by the subsequent
stages in the pipeline. The class of computations at each stage are simple data
parallel operations applied on all image pixels such as point-wise and stencil
computations.  Figure~\ref{fig:hdag} shows the computational DAG associated with
the Harris Corner Detection (HCD) benchmark. As the name indicates, HCD is a corner
detection algorithm, commonly used in computer vision space.
Table~\ref{tab:hcd} shows the computations at each stage of the DAG.
The source code for HCD benchmark in PolyMage DSL, whose compiler infrastructure we use
in this paper,
can be obtained at the PolyMage  GitHub repository~\cite{polymagebench}.  
If the computations in HCD  are expressed in C/C++,
then there will be a two dimensional loop associated with each stage of the DAG.
Further, these loops occur in some topologically sorted order of DAG nodes.
Thus, the rich structure in the application gets lost in the resulting C/C++
code. For example, it is hard to infer that pixels output from one stage can be
streamed to the following stage and the following stage can start computations
once it receives enough number of pixels. This observation leads to an extremely
efficient pipelined hardware architecture for the whole computational DAG and is
exploited in PolyMage-HLS compiler as in other DSL compilers for FPGAs. In this
paper, we use the fact that it is easy to infer the computations on pixels at
each stage of the DAG and further these computations are applied homogeneously on
all the pixels at the corresponding stage, to arrive at efficient range
analysis algorithms based on interval arithmetic and Satisfiability Modulo 
Theory (SMT) solvers.  It would be almost impossible to do
this if the design is expressed directly in Verilog/VHDL; and probably require
complex program analysis if we have to to achieve this on C/C++ programs as is
the case in HLS frameworks.

\subsection{Problem Description and Contributions}
The data at each stage of an image processing pipeline is represented using
a parametric fixed-point data type $\left(\alpha, \beta\right)$, where $\alpha$ 
and $\beta$
denote the number of bits used to represent integral and fractional parts.  The
objective is to minimize $\alpha$  and $\beta$ at each stage while maintaining
an application specific quality metric. The optimal value of $\alpha$ at a stage
depends on the range of values produced; whereas the optimal value of $\beta$
depends on how precision impacts the quality metric.

Range analysis which is required for estimating the integral bitwidth requirement
is a well studied problem in literature. There are several works
based on variants of interval and affine arithmetic~\cite{cong09fccm, vakili13tcad, 
zhang10jsip, stephenson00sigplan, lee06tcad, mahlke01tcad}.
The benchmarks considered in these works, such as FIR filter, Discrete Cosine
Transform, Polynomial Evaluation etc.  are mainly from the signal processing domain 
and their code size and complexity is small. These techniques are not
easily adaptable for image processing pipelines  when expressed in Verilog/VHDL,
HLS C/C++ etc. due to the large number of pixel signals present at each stage
and multiple such stages in an application. 

The first main contribution of our paper is an interval arithmetic based range analysis 
technique in the DSL compiler which exploits the fact that the computations on all
the pixels at a given stage is homogeneous to do a combined range analysis. The
second main contribution of our paper is a range analysis framework in the DSL compiler 
wherein any interval and affine arithmetic-like analysis can be incorporated with ease.

Apart from interval arithmetic based approaches, which cannot handle certain
kind of operations like divisions, techniques using powerful SMT solvers have
been proposed in the literature~\cite{ kinsman10}. However, they are applied on
extremely small benchmarks involving 2 to 3 equations. The third main
contribution of this paper is that, we  propose a range analysis technique using
SAT solvers and apply it on large benchmarks such as Optical Flow involving few
tens of DAG stages not to speak of large number of pixel signals and complex
computations in the DAG structure. This is primarily possible because our
analysis is based on the DSL specification of the benchmark as against a HDL or
C/C++ specification. Further, we show that in iterative algorithms such as
Optical Flow, conservative estimates of interval analysis will have a
debilitating effect with the increase in the iterations making them unusable in
practice; and we have to resort to SMT solvers to get accurate range estimates.

The fourth main contribution of this paper is a simple greedy heuristic search
technique for precision analysis to determine the number of bits required for
representing fractional bits at each stage of the pipeline. Finally, we present
a thorough experimental study comparing the effectiveness of interval, SMT
solver and profile guided approaches with respect to power, area and speed on
large image processing benchmarks. We would like to highlight that all the
previous studies involve very small benchmarks. 

We implement and evaluate our automatic bitwidth analysis approach in PolyMage
compiler infrastructure \cite{mullapudi2015asplos, chugh16pact}. With the PolyMage DSL, FPGAs are targeted by
first generating High-Level Synthesis (HLS) code after a realization of
several transformations for parallelization and reuse; the HLS code is
subsequently processed by a vendor HLS suite (Xilinx Vivado in the case of
PolyMage). There have been several recent DSL efforts that target FPGAs for image
processing; these include Darkroom~\cite{darkroom},
Rigel~\cite{rigel}, Halide~\cite{halide17hls}, HIPAcc~\cite{hipacc16fpga} and
PolyMage-HLS~\cite{chugh16pact}. While these works
have addressed several challenges in compiling DSL to FPGAs, none of them
have studied the issue of exploiting application-dependent
variable fixed-point data types for power and area savings. HiPAcc
goes to the extent of providing pragmas for specifying bitwidths of
variables, but no automatic compiler support for it.

\begin{table}[t]
\begin{minipage}[b]{0.38\linewidth}
\includegraphics[scale = 0.8]{./graphs/harris_annotated_dag}
\captionof{figure}{DAG representation of the Harris Corner Detection (HCD) algorithm.}
\label{fig:hdag}
\end{minipage}\hfill
\begin{minipage}[b]{0.58\linewidth}
%\centering 
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{r  |r} 
\toprule
%\hline\hline %inserts double horizontal lines
Stage  & Computation \\  % inserts table
%heading
\hline % inserts single horizontal line
$I_x$ &  $\frac{1}{12}\left[ \begin{smallmatrix} -1 & 0 & 1 \\ -2 & 0 & 2 \\ -1 & 0& 1\end{smallmatrix} \right]$  \\ % inserting body of the table
$I_y$ &  $\frac{1}{12}\left[ \begin{smallmatrix} -1 & -2 & -1 \\ 0 & 0 & 0 \\ 1 & 2& 1\end{smallmatrix} \right]$  \\
$I_{xx}$ &  $I_x\left(i,j\right) I_x\left(i,j\right)$ \\
$I_{xy}$ &  $I_x\left(i,j\right) I_y\left(i,j\right)$  \\
$I_{yy}$ &  $I_y\left(i,j\right) I_y\left(i,j\right)$  \\
$S_{xx}$ &  $A=\left[ \begin{smallmatrix} 1 & 1 & 1 \\ 1 & 1 & 1 \\ 1 & 1 & 1\end{smallmatrix} \right]$\\
$S_{xy}$ &  $A$\\
$S_{yy}$ &  $A$\\
$det$ &  $S_{xx}\left(i,j\right) S_{yy}\left(i,j\right)-S_{xy}\left(i,j\right) S_{xy}\left(i,j\right)$\\
$trace$ &  $S_{xx}\left(i,j\right)+S_{yy}\left(i,j\right)$\\
$Harris$ &  $det\left(i,j\right) - 0.04 ~trace\left(i,j\right) trace\left(i,j\right)$\\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
%}%
\caption{Summary of computations in HCD benchmark.}
\label{tab:hcd}
\end{minipage}
\end{table}


The rest of this paper is organized as follows. Related work is discussed in
Section~\ref{sec:related-work} and the necessary background is provided in
Section~\ref{sec:background}. Section~\ref{sec:bitwidth} presents in detail the
main contributions of this paper. 
Experimental evaluation is
presented in Section~\ref{sec:experiments} and  conclusions are presented in
Section~\ref{sec:conclusions}.
%
%
%\input{files/pointwise_algorithm}
%


==> files/my_abstract.tex <==
While recent Domain Specific Languages have eased FPGA programming, low level
details are generally ignored. Since most of the attention is given to
throughput improvement, power and area savings are taken for granted and are
thought of as a virtue of using FPGAs. FPGAs are a promising platform for
implementation of ~high-compute-algorithms in low power scenarios with ~less-
overhead-expenses(ASICs) and the low level details like bitwidths of variables
become important here. Image processing is a very common such application. While
it's convenient to use floating point data types for real-value programs, there
exists significant slack in the bitwidth representation, leading to inefficient
implementations. 

Our technique allows the programmer to specify his algorithm in
float and get bitwidth customized implementation automatically.

==> files/pointwise_algorithm.tex <==
% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
\algnewcommand{\IfThenElse}[3]{% \IfThenElse{<if>}{<then>}{<else>}
   \algorithmicif\ #1\ \algorithmicthen\ #2\ \algorithmicelse\ #3}
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
%\algtext*{EndSwitch}%
\algtext*{EndCase}%

\begin{algorithm*}[t]
\caption{Integral bit-width analysis algorithm applied at each stage of the DAG in topological sorted order. }\label{alg:precision}
\begin{algorithmic}[1]
\Procedure{ComputeBitwidth}{$e$}%\Comment{The g.c.d. of a and b}
\If{\textit{e->data} $==$ leaf\_operand} 
  \State \Return \textit{e->bitwidth} \Comment{ Bitwidth is a 3-tuple $(\low{e},\high{e},\alpha)$ already computed for leaf nodes.}
\Else \Comment{$[\low{e}, \high{e}]$ is the range and $\alpha$ is the number bits required to represent the range.}
  \State $op \gets$ \textit{e->operator}
  \State $(\low{x},\high{x},\alpha_1) \gets$ \Call{ComputeBitwidth}{\textit{e->left}}
  \State $(\low{y},\high{y},\alpha_2) \gets$ \Call{ComputeBitwidth}{\textit{e->right}}
    \Switch{($op$)}
    \Case{+ :}
     $[\low{z},\high{z}] \gets [\low{x}+\low{y}, \high{x}+\high{y}]$ 
    %\State $\beta_{z} \gets \max(\beta_x,\beta_y)$
    \EndCase
    \Case{- :}
    $[\low{z},\high{z}] \gets [\low{x}-\high{y}, \high{x}-\low{y}]$
    %\State $\beta_{z} \gets \max(\beta_x,\beta_y)$
    \EndCase
    \Case{* :}
     $[\low{z},\high{z}] \gets [\min(\low{x}\low{y}, \low{x}\high{y}, \high{x}\low{y}, \high{x}\high{y}), \max(\low{x}\low{y}, \low{x}\high{y}, \high{x}\low{y}, \high{x}\high{y})]$
    %\State $\beta_{z} \gets \beta_x+\beta_y$
    \EndCase    
    \Case{/ :} 
    \IfThenElse {$0 \not \in [\low{y}, \high{y}]$}
      {$[\low{z},\high{z}] = [\low{x}, \high{x}] * [1/\high{y}, 1/\low{y}]$}% ...then...
      {$[\low{z},\high{z}] = [-\infty, +\infty]$}% ...else...
    \EndCase
    \iffalse
    \Case{\ \^{} :} 
    \State $n = \low{y} = \high{y}$ \Comment{Exponentiation operation is defined for constant value powers only.}  
    \If{$n$ is odd} \State $[\low{z},\high{z}] = [\low{x}^n, \high{x}^n ]$
    \ElsIf {$\low{x} \geq 0$} \State $[\low{z},\high{z}]  =  [\low{x}^n, \high{x}^n ]$
    \ElsIf {$\high{x} < 0$} \State $[\low{z},\high{z}]  =  [\high{x}^n, \low{x}^n ]$ 
    \Else \State $[\low{z},\high{z}]  = [0, max\{\low{x}^n, \high{x}^n\} ]$
    \EndIf 
    \EndCase
    \fi
    \iffalse
    \Case{$\verb|^|$ :} \State $ad$
    \EndCase
    \fi
    \iffalse
    \If{$\low{z}>0$ or $\high{z} <0$}    
    \State $[\low{z},\high{z}] = [\min(\low{x}\mbox{\small/}\low{y}, \low{x}\mbox{\small/}\high{y}, \high{x}\mbox{\small/}\low{y}, \high{x}\mbox{\small/}\high{y}), \max(\low{x}\mbox{\small/}\low{y}, \low{x}\mbox{\small/}\high{y}, \high{x}\mbox{\small/}\low{y}, \high{x}\mbox{\small/}\high{y})]$
    \Else 
    \State $[\low{z},\high{z}] = [\low{p}, \high{p}]$ \Comment{The range $[\low{p}, \high{p}]$ is estimated by program profiling.}     
	\EndIf 
    \fi
    %\State $\beta_{z} = \beta_x + \ceil{\log_2{\high{y}}} + t $    \Comment{The configurable parameter $t$ controls accuracy and can be set to some default value.}
    
    \EndSwitch
    
	
    \State $\alpha_{z} \gets \begin{cases}
    \max(\ceil{\log_2(\ceil{|\low{z}|})},\ceil{\log_2(\floor{|\high{z}|}+1)})+1,& \text{if } \low{z} <0\\
    \ceil{\log_2(\floor{\high{z}}+1)},              & \text{otherwise}
\end{cases}$
    \State \Return $(\low{z},\high{z},\alpha_z)$
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm*}

==> files/precision-algorithm.tex <==
\iffalse
The following files have to be included in paper.tex
      \usepackage{amsmath}
      \usepackage{algorithm}
      \usepackage{algpseudocode}
\fi
%
% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
%\algtext*{EndSwitch}%
\algtext*{EndCase}%
%
\begin{algorithm}
\caption{Precision analysis algorithm applied at stages performing point-wise computations.}\label{alg:precision}
\begin{algorithmic}[1]
\Procedure{EvaluatePrecision}{$e$}%\Comment{The g.c.d. of a and b}
\If{\textit{e->data} $==$ operand} 
  \State \Return \textit{e->type}
\Else %{\textit{e->data} == operator}
  \State $op \gets$ \textit{e->operator}
  \State $T' \gets$ \Call{EvaluatePrecision}{\textit{e->left}}
  \State $T'' \gets$ \Call{EvaluatePrecision}{\textit{e->right}}
    \Switch{($op$)}
    \Case{+ :}
      \State $T^r_I \gets \max(T'_I,T''_I)+2$
      \State $T^r_F \gets \max(T'_F,T''_F)$
      %\State \Return $T^r$
    \EndCase
    \Case{- :}
      \State $T^r_I \gets \max(T'_I,T''_I)+2$
      \State $T^r_F \gets \max(T'_F,T''_F)$
      %\State \Return $T^r$
    \EndCase
    \Case{* :}
      \State $T^r_I \gets T'_I + T''_I$
      \State $T^r_F \gets T'_F + T''_F$
      %\State \Return $T^r$
    \EndCase    
    \Case{/ :}
      \State $T^r_I \gets T''_I+T'_F$
      \State $T^r_F \gets T''_F+T'_I$
      %\State \Return $T^r$
    \EndCase
    \EndSwitch
    \State \Return $T^r$
\EndIf
\EndProcedure
\iffalse
\Statex
\Statex
\Procedure{Main}{}\Comment{Given a DAG (G)}
\State topologicalSort($G,stack$) 
\While{isEmpty($stack$) $==$ $False$}
\State $node \gets$ pop($stack$)
\State $e \gets$ fetchExpressionTree($node$)
\State \Call{EvaluatePrecision}{$e$}
\EndWhile
\EndProcedure
\fi

\end{algorithmic}
\end{algorithm}


==> files/profile.tex <==
\section{Profile-Driven Analysis}
\label{sec:profile}
Profile-driven analysis can be used to accomplish two tasks. First, the 
worst-case integral bit-width lengths  at various stages obtained via static 
analysis can be improved. Second, the number of fractional bits required at 
each stage can be estimated using an application-specific quality metric.  
However, the bit-width  requirements estimated at each stage using profiling 
technique naturally depends on the sample input images. Based on the 
analysis done by Torralba et al. \cite{torralba2003statistics}, we 
hypothesize that the images taken from a certain domain, like for example 
{\it nature}, has similar properties, and hence the bit-width estimates can 
be carried over to other images drawn from the same domain.
\input{files/flow}
%
\subsection{Integral Bits}
The number of integral bits required at a stage $i$ denoted as $\alpha_i$  can
be obtained by running the input PolyMage program on a sample  distribution of
input images. Let $\alpha_i^s$ be the maximum number of bits  required by stage
$i$ to represent a pixel from an image sample $s$. Then  the average number of
bits $\alpha_i^{avg}$ required based on a sample set  $S$ is $\sum_{s\in S}
\alpha_i^s/|S|$. Similarly, the worst-case number of  bits $\alpha_i^{max}$
required is $max_{s\in S} \alpha_i^s$. We can either  use $\alpha_i^{avg}$ or
$\alpha_i^{max}$ as estimates for $\alpha_i$. Even if the estimate does not suit
certain images, in many application  contexts, using saturation mode arithmetic
results in satisfying the desired  output quality metric. Let $\alpha_i^{sa}$ be
the integral bit-width  estimation obtained for stage $i$ through static
analysis. For the benchmark programs we have considered, affine analysis show some 
improvements in the range estimates, but it amounts to same bit-width requirement as
with interval analysis. Hence,  throughout the rest of the paper, when
we refer to static analysis it means interval analysis only.

For our experimentation, we used a subset of 200 randomly chosen images from 
the Oxford Buildings dataset~\cite{oxfordimages} consisting of 5062 images. 
The set of 200 images is partitioned into two equal halves: training and 
test sets. The training set is used to obtain estimates of integral 
bit-widths at various stages through profiling. The test set is used to 
evaluate the effectiveness of the bit-width estimates obtained for quality 
and power. Figure~\ref{fig:hs} shows the average cumulative distribution of 
the bit-width required by the integral part of the pixels in stages $I_x$
and $I_{xy}$  of the HCD program on the training data set. 
\iffalse
The x-axis of the graphs represent the bit-width requirement of the integral 
part, and y-axis represents the percentage of pixels, averaged across test 
images, that can be represented within a given bit-width.  
\fi
For example, from Figure~\ref{fig:hs1}, we can infer that in stage $I_x$,  
95\% of the pixels require less than 5 bits, and all pixels (100\%) can be represented using 8 bits.
\iffalse  
Since 
stages $I_x$ and $I_y$ are of similar computational nature, we plot the 
histogram for only $I_x$.  Similarly, among $I_{xx}$, $I_{xy}$ and $I_{yy}$, 
we plot for $I_{xy}$ in Figure~\ref{fig:hs2}, and from stages $S_{xx}$, 
$S_{xy}$ and $S_{yy}$, we plot for $S_{xy}$ in Figure~\ref{fig:hs3}.  
Figures~\ref{fig:hs4},~\ref{fig:hs5} and~\ref{fig:hs6} correspond to {\it 
det}, {\it trace} and {\it Harris} stages respectively.
\fi  
Table~\ref{tab:bitTableHCD},~\ref{tab:bitTableUSM_DUS} shows the bit-width estimates obtained from 
static and profile-driven analyses.
%
\begin{table*}[h!]
    \footnotesize
    \caption{Comparison of integral bitwidth estimates using interval, \smtra, 
    and profile-guided analyses for HCD and DUS. Fractional bitwidth estimates are also provided.}
    %\vskip 5pt
    \label{tab:bitTableHCD}
\centering
    %\resizebox{\linewidth}{!}{%
        \begin{tabularx}{1.07\linewidth}{c | c c c c c c c c c}
        \toprule
        & &&&&HCD&&&&\\
        Stage&Img&I$_x$,I$_y$&I$_{xx}$,I$_{yy}$&I$_{xy}$&S$_{xy}$&S$_{xx}$, S$_{yy}$&det&trace&harris\\
        \midrule
        $Z3$ &          8&8&13&14&17&16&33&17&\bf{33}\\
        $\alpha^{IA}$ & 8&8&13&14&17&16&33&17&34\\
        \midrule
        $\alpha^{maxP}$& 8&8&13&14&17&16&30&17&29\\
        $\alpha^{avgP}$& 8&8&13&14&17&16&29&17&29\\
        $\beta$ & 8&5&4&4&3&3&1&1&1       \\
        \bottomrule
        \end{tabularx}
        %}%
\end{table*}
%
\begin{table*}[h!]
    \footnotesize
    \caption{Comparison of bit-width estimates using profiling technique and static analysis for USM and DUS.}
    \vskip 5pt
    \label{tab:bitTableUSM_DUS}
\centering
    %\resizebox{\linewidth}{!}{%
        \begin{tabularx}{1.07\linewidth}{c | c c c c c | c c c c c }
        \toprule
        &&&USM&& &&&DUS&&\\
        Stage&Img&blur$_x$&blur$_y$&sharpen&mask&Img&D$_x$&D$_y$&U$_x$&U$_y$\\
        \midrule
        $Z3$ &8&8&8&10&9 &8&8&8&8&8\\
        $\alpha^{IA}$  &8&8&8&10&9 &8&8&8&8&8\\
        \midrule
        $\alpha^{maxP}$ &8&8&8&10&9 &8&8&8&8&8\\
        $\alpha^{avgP}$ &8&8&8&10&9 &8&8&8&8&8\\
        $\beta$  &0&2&3&4&4  &0&3&6&8&10\\
        \bottomrule
        \end{tabularx}
        %}%
\end{table*}
%
As can be noted from 
Table~\ref{tab:bitTableHCD}, the bit-width estimates from $\alpha^{avg}$ 
and $\alpha^{max}$  measures are the same for all stages 
except for the {\it det} stage.  
The estimates from the static analysis match the profile estimates except 
for the {\it det}, {\it trace} and {\it harris} stages. In general, we 
expect the profile estimates to be better for stages that occur deeper in 
the pipeline. Note that the profile estimates also indicate the limit to 
which the static analysis techniques can be improved by using more powerful 
approaches. Profile information can be easily 
obtained by executing the HLS C++ program directly without the need for a 
heavy weight circuit simulation.
%
\begin{figure}[hb]
%\captionsetup[subfigure]{labelfont=bf,textfont=normalfont}
\centering
\resizebox{\columnwidth}{!}{%
  \harrisHist
  }%
    \vskip 5pt
\caption{Cumulative distribution of pixels with respect to maximum integral bit-width length at 
 stages $I_x$ and $I_{xy}$ of the HCD program.}
\label{fig:hs}
\end{figure}
\subsection{Fractional Bits ($\beta$) Analysis}
The number of fractional bits $\beta_i$ required at a stage $i$ depends on the
application and cannot be estimated in an application independent way as is
the case with the integral bits analysis. Estimating the optimal number of
fractional bits at each stage for a given application metric turns out to be a
non-convex optimization problem in most cases and hence we propose a simple 
heuristic search technique that requires very few profile passes. 

In the profiling technique, we fix the number of integral bits required at each 
stage based on static or profile-driven analysis and increase the precision 
$\beta$ uniformly across all the stages. For each value $\beta$, we estimate 
the application-specific error metric. For the HCD benchmark, the error 
metric is the percentage of mis-classified corners when compared to a design 
which uses sufficiently long integral and fractional bits. We can reach an 
optimal $\beta$ for a given error tolerance via binary search. Then we make
a single pass on the stages of the DAG in reverse topologically sorted order.
At each stage $I$, we do a binary search on the number of fractional bits 
required, $\beta_I$, starting from the initial estimate $\beta$ while 
retaining the application specific quality requirement. Figure~\ref{fig:flow}
summarizes the proposed bitwidth analysis framework.
%
\iffalse
Figure~\ref{fig:uniformbeta} shows the average percentage of pixels correctly 
classified by the HCD program on the test image set by varying the 
fractional bits uniformly across all the stages while fixing the integral 
bit-width estimates obtained via profiling ($\alpha_i^{avg}$). It also 
contains estimates of power consumption with varying fractional bits for the 
Xilinx ZedBoard FPGA.
It can be noted from the graph that the fractional bits do not affect the 
accuracy of corner classification, and we thus get more than 99\% 
accuracy even with zero fractional bits. From this graph, we infer that one 
can obtain close to 100\% accuracy by using 10 fractional bits uniformly 
across all the stages. We then make a backward pass on the stages of the
HCD program to drop the fractional bits further without any significant loss
in accuracy and the column corresponding to $\beta^{avg}$ in 
Table~\ref{tab:bitTableHCD} shows the final fractional bitwidths.

Table~\ref{tab:HCDresults} shows the accuracy, power 
and area metrics obtained when the HCD program is applied on the test data
using float, bit-widths from static and profile analysis. It can be noticed 
that by using bitwidths from static analysis, we obtain 99.999\% accuracy with
a power consumption of 0.263~W. The power savings are 
3.8$\times$ lower when compared with the baseline PolyMage-HLS compiler 
  generated code using float data type. With respect to area, the number of 
  slices used, the savings over using float is around 6.2$\times$.  The 
  number of DSPs used by the fixed-point and floating-point designs 12
  and 112 respectively. Similarly, the number of BRAM units used by the 
  fixed-point and floating-point designs are 14 and 12 respectively.
  The last 3 columns of the Table~\ref{tab:HCDresults} show the maximum
  frequency of operation by different designs and it can be noted that can
  run at a higher frequency achieving better throughput while consuming lesser
  power.
   \begin{table*}[htb]
    \footnotesize
    \caption{Quality, post place and route power, area and throughput metrics for the HCD program using float and, bit-widths estimated using static analysis and profiling techniques.The fractional bits used are from Table~\ref{tab:bitTableHCD}.}
    \vskip 5pt
    \label{tab:HCDresults}
\centering
    \harrisRes
\end{table*}
\fi


==> files/related-work.tex <==
\section{Related Work}
\label{sec:related-work}
Besides PolyMage~\cite{mullapudi2015asplos},  Rigel~\cite{rigel},
Darkroom~\cite{darkroom}, HIPAcc~\cite{membarth16tpds}, and
Halide~\cite{kelley13pldi} are other recent domain-specific languages (DSL) 
for image processing pipelines.  Among them, PolyMage, Rigel, HIPAcc, and
Darkroom compilers can generate hardware designs targeting FPGAs, and none of
these currently optimize designs using bitwidth analysis.

There are several works on bitwidth estimation in digital signal processing
applications ~\cite{TEMA352, vakili13tcad, cong09fccm, lee06tcad,
zhang10jsip}. However, these techniques are not scalable and can only be applied to small circuits
like low degree polynomial multiplications, 8x8 discrete cosine transform
computation etc. which contain very few signals in the order of 10s and 100s.
Whereas the techniques proposed in this paper exploits both the image processing
domain and the PolyMage-HLS compilation framework to do interval analysis on
large image processing pipelines wherein each pixel at every stage of the pipeline
constitutes a signal. Further, there are a class of iterative algorithms such as
optical flow wherein errors in range estimation accumulate across iterations making
the analysis in essence useless. In this work, we show
how we can use SMT solvers to get accurate range estimates and thus contain errors
across iterations. Kinsman and Nicolici~\cite{kinsman10} proposed a SMT solver based
approach, however, they evaluated their approach on small signal processing
applications involving less than 10 signals. The SMT solver based approach proposed 
in the current work handles large image processing applications which are iterative
in nature with potentially thousands of pixel signals being processed in each 
iteration. 

%

Usually, range analysis (integer bits) and precision (fraction bits)
analysis are performed separately. For precision analysis, there are
heuristic search~\cite{vakili13tcad, nguyen11precision} based approaches which try to minimize circuit area and power while satisfying  constraints on Signal-to-Noise 
ratio. The time complexity of these algorithms is usually very high and hence 
impractical to use in large image processing pipelines. Whereas, the greedy heuristic 
algorithm we proposed in this paper runs in linear time with respect to the number of stages
present in the image processing pipeline and is independent of the image dimensions.
Overall, ours is the first extensive study on the
application of practical range and precision analyses in image processing 
applications, and their impact on power and area savings.


\iffalse
We study the effectiveness of interval
analysis in estimating integral bitwidths and compare it with the estimates
obtained via profile-driven analysis. The interval analysis algorithm nicely
fits into the data flow analysis framework used in all modern compilers. For
precision analysis to estimate fractional bits, we use uniform bitwidths
across all the stages and then use simple linear or binary search algorithms
to arrive at a suitable bitwidth meeting an application-specific quality
criteria.
\fi


Mahlke et al.~\cite{mahlke01tcad} proposed a data flow analysis based approach
for bitwidth estimation of integral variables in the PICO (Program-in Chip-out)
system for synthesizing hardware from loop nests specified in C.  Along the same
lines, Gort and Anderson~\cite{anderson13range} proposed a range analysis
algorithm in the LegUp HLS tool. Their  range analysis algorithm is designed
over the LLVM intermediate representation and is implemented as an LLVM 
analysis pass. On the other hand, the interval arithmetic based range 
analysis algorithm we will propose works at
the DSL level and furthermore, the  proposed compilation framework permits 
the
usage of any other range analysis algorithm nearly in a plug-and-play 
manner; this can otherwise require significant effort in order to make it 
into a compiler analysis pass.

The integral bitwidth analysis algorithm due to Budiu et 
 al.~\cite{budiu00europar} is similar to the previous work but uses a
 different data flow analysis formulation.
Stephenson et al.~\cite{stephenson00sigplan} performs integer bitwidth
 analysis through range propagation, again using a data flow analysis
 framework.
 Tong et al. \cite{tong00customfp} proposed the usage of variable
 bitwidth floating-point units, which can save power for applications that
 do not require the full range and precision provided by the standard
 floating-point data type.
  Sampson et al. \cite{sampson11enerj} proposed
 EnerJ, an extension to Java that supports approximate data types and
 computation.  However, fixed-point data types and the associated approximate
 operations are not considered in EnerJ. On the contrary, PolyMage DSL can be
 enhanced by using the approximate data types as proposed by EnerJ.

Approximate computing has a rich body of
literature~\cite{mittal16approxsurvey, ramani15approx, han13approx}.
However, our context of
domain-specific automatic HLS compilation is unique. Depending on the output
quality and the application in question, our approach could either be seen
as exploiting customized precision or leveraging approximate computing.
In addition to customized precision, we can potentially use approximate
arithmetic operations \cite{kahng12adder, liu14multiplier} in the various
stages of computation.


==> files/running-example-smt.tex <==
\subsubsection{Example with Horn-Schunck Optical Flow}\label{sec:smt_running_example}
\iffalse
Comment start
\\ 
So, just for the terminology, I'll say that the initial input variables (stage 0) are fundamental variables and all other variables introduced in successive stages are derived variables and can be written completely in terms of stage0 vars when all correlations are preserved. Breaking correlations at a stage means that the output variables of that stage are now new fundamental vars (which i used to call dummy vars). Also, now we can also have a hybrid way of solving, where we
break the correlations at some stages, not all. And the question is how to choose those stages. 
As of now, i tried various ways, and none worked for HCD.
\\
comment end
\fi

In Horn-Schunck optical flow, all stencils are 3x3. Since this optical flow solves for the correct motion vectors in an iterative manner, the DAG gets pretty huge just after 3-4 iterations and to be able to use Z3, we break the correlations before every stencil stage. We do this because otherwise every stencil stage will require at-least 9 input variables from the parent and breaking correlations at their parent significantly reduces the total number of variables and their degree. Hence, 9 fundamental variables are created at the parent of each stage. 

The DAG is shown in figure \ref{fig:hsof_dag}. From this DAG, the code for SMT analysis using Z3 python API is generated as shown in listing \ref{list:of_z3}.


\ofsmtcode



\iffalse
\begin{figure}
\centering
\includegraphics[scale = 0.8]{./graphs/hs_of_dag}
\captionof{figure}{DAG representation of the Horn-Schunck Optical Flow algorithm.}
\label{fig:hsof_dag}
\end{figure}
\fi

\iffalse
\begin{figure}
\includegraphics[width=4cm]{images/HS-OF-DAG}
\caption{Horn-Schunck Optical Flow DAG}
\label{fig:hsof_dag}
\end{figure}
\fi

==> files/smt-top.tex <==
\section{Motivation SMT}
(Placeholder for Motivation on Z3 approach)
\\
\\
(Discussion on how the ranges are calculated is here)
\\
\\
<<<<<<< HEAD
The range(bitwidth) for each stage is solved in the topologically sorted order as per the image processing DAG. The input to any DAG is an image. We consider this as the first stage and the range associated with the variables in this stage is (0,255). This, in turn is the input to the second stage and also a constraint. Generalising, each node in the dag is a stage and parents to that node add their constraints to the solver which are used for solving the range for this stage.
The range for a stage is solved in the following manner. Depending on the nature of the stage, an expression, say $exp$, can be obtained which specifies it's operation on the input(s). The goal is to find the minimum and the maximum value this expression can take. (The expression can be non-linear etc.. The other optimisers may not give global min/max. But SMT does give a definite upper or lower bound). This is where Z3 is used. For finding the upper bound, we start with a sufficiently large negative value, say $maxVal$, and check the satisfiability of the equation $exp > maxVal$. If $there_exist$ any assignment of the variables in the $exp$ for which this is true, the solver returns $sat$ which means satisfiable. In such a case the value of $maxVal$ is reduced and this procedure is iteratively repeated until we reach a point on the real number line such that the solvers $sats$ on the left epsilon neighbourhood and $unsats$ on the right epsilon neighbourhood of that point. Epsilon is an input parameter and should be less than 1. Similarly we solve for the minimum value the expression can take. From the min and max values, the integeral bitwidth requirement for this stage is calculated as in equation ?. (I have to add the math expression here for calculating bitwidth from range).
=======
The range(bitwidth) for each stage is solved in the topologically sorted order as per the image processing DAG. The input to any DAG is an image. We consider this as the first stage and the range associated with the variables in this stage is (0,255). This, in turn is the input to the second stage and also a constraint. Generalizing, each node in the dag is a stage and parents to that node add their constraints to the solver which are used for solving the range for this stage.
The range for a stage is solved in the following manner. Depending on the nature of the stage, an expression, say $exp$, can be obtained which specifies it's operation on the input(s). The goal is to find the minimum and the maximum value this expression can take. (The expression can be non-linear etc.. The other optimizers may not give global min/max. But SMT does give a definite upper or lower bound). This is where Z3 is used. For finding the upper bound, we start with a sufficiently large negative value, say $maxVal$, and check the satisfiability of the equation $exp > maxVal$. If $there_exist$ any assignment of the variables in the $exp$ for which this is true, the solver returns $sat$ which means satisfiable. In such a case the value of $maxVal$ is reduced and this procedure is iteratively repeated until we reach a point on the real number line such that the solvers $sats$ on the left epsilon neighbourhood and $unsats$ on the right epsilon neighbourhood of that point. Epsilon is an input parameter and should be less than 1. Similarly we solve for the minimum value the expression can take. From the min and max values, the integral bit-width requirement for this stage is calculated as in equation ?. (I have to add the math expression here for calculating bitwidth from range).
>>>>>>> 4880d77b8a79889eccf4baecfae4af205af77527

The important point here is that the constraints and the expressions are stored symbolically and the information about the ancestors of a node is available to the node and this captures the correlations between the variables in the expression of the current node and this results in a tight bound. But it has it's own price. The complexity of the DAG can depend on many factors such as it's depth, degree of expressions in the stages, etc. As the complexity increases, it becomes harder and confusing
for Z3 to check the satisfiability and it severely affects the runtime and capability of Z3 to solve. For some cases, it may also return $unknown-solution$.

The input image variables are the fundamental variables and all other variables of stages are derived from them. This keeps all the correlations intact. As we move down the DAG, each derived variable becomes either higher in degree or higher in total number of unknowns. After a while z3 starts to fail. To deal with this problem, we need to keep the degree and unknowns of derived variables under control. For this we break the correlations at certain stages and introduce new fundamental
variables there. This is done by declaring completely new variables and assigning them the correct range of that stage and these flow down the dag now.

Stage 0 is the input stage and the total number of variables are equal to the input image size. To further reduce the total number of variables flowing in the system, as a first step, we calculate the minimal variables required from stage0 for full correlation capture. So, in essence, only those variables are selected at stage0 which are just enough to produce one output at the last stage. This is calculated by projecting the requirement bottom up starting from the last stage. Without loss of generality, given a 2-D matrix of size MxM, the dimension remains same if point-wise operation is applied to it. If a stencil of dimension say NxN and stride S is applied to it, then the size reduces to $floor((M-((N-1)/2))/S) \ \ X \ \ floor((M-((N-1)/2)/S)$ assuming N is odd. Using these equations, the minimum input variable matrix size can be calculated for any arbitrary DAG as after all the reductions, in whatever order, the final size should be 1. We do this compulsorily for every DAG.

For complex computer vision pipelines such as optical flow, we still have to break correlations at certain places. In section ?, this is taken as a running example to understand the code and the framework. 
\\
(Next file is general-framework-smt.tex)
